Predicting the Big Five Personality Traits in Chinese Counselling Dialogues Using Large Language Models

Accurate assessment of personality traits is crucial for effective psycho-counseling, yet traditional methods like self-report questionnaires are time-consuming and biased. This study exams whether Large Language Models (LLMs) can predict the Big Five personality traits directly from counseling dialogues and introduces an innovative framework to perform the task. Our framework applies role-play and questionnaire-based prompting to condition LLMs on counseling sessions, simulating client responses to the Big Five Inventory. We evaluated our framework on 853 real-world counseling sessions, finding a significant correlation between LLM-predicted and actual Big Five traits, proving the validity of framework. Moreover, ablation studies highlight the importance of role-play simulations and task simplification via questionnaires in enhancing prediction accuracy. Meanwhile, our fine-tuned Llama3-8B model, utilizing Direct Preference Optimization with Supervised Fine-Tuning, achieves a 130.95\% improvement, surpassing the state-of-the-art Qwen1.5-110B by 36.94\% in personality prediction validity. In conclusion, LLMs can predict personality based on counseling dialogues. Our code and model are publicly available at \url{https://github.com/kuri-leo/BigFive-LLM-Predictor}, providing a valuable tool for future research in computational psychometrics.

==> sec/1.introduction.tex <==
\section{Introduction}
\label{sec:intro}

% \YY{Paragraph 1 \& 2: Why is the problem important? Why is the problem difficult?}

% Understanding clients' personality traits is paramount for effective psychological counseling. \YY{Logical gap between two sentences, The subjects of the two sentences do not match} 
% Personalized advice tailored to these traits can significantly enhance the quality of counseling~\cite{gordon2002said,anestis2021personality}. 
Understanding clients' personality traits is crucial for effective psychological counseling, as personalized advice tailored to these traits can significantly enhance the quality of counseling~\cite{gordon2002said,anestis2021personality}.
% Despite its importance\YY{Potential misunderstanding, what does ``its'' refer to, and what is the connection between ``importance'' and ``challenge''}, assessing personality traits accurately remains fraught with challenges. 
However, efficiently and effectively assessing personality traits from counseling dialogue remains challenging.
% Traditional tools like the Big Five Inventory (BFI)~\cite{john1991big}, grounded in Item Response Theory~\cite{baker2001basics,reise2009item,embretson2013item}, \lizhi{require} clients to complete extensive questionnaires. 
Traditional tools like the Big Five Inventory (BFI)~\cite{john1991big}, grounded in Item Response Theory~\cite{baker2001basics,reise2009item,embretson2013item}, require clients to complete extensive questionnaires.
% This process is not only time-consuming but also \lizhi{influenced by} subjective biases and social desirability effects\YY{TODO:add cite to support this}, undermining \lizhi{the comprehensive measurement of personality}~\cite{chernyshenko2001fitting,khorramdel2014measuring,mccrae2007observer}~\YY{TODO: Move some cites to previous sentence}. 
Participation in self-reporting makes the process not only time-consuming but also influenced by subjective biases and social desirability effects~\cite{chernyshenko2001fitting}, undermining the comprehensive measurement of personality~\cite{mccrae2007observer,khorramdel2014measuring}.
% Consequently, the quest for an automatic, unbiased method to assess personality traits without direct client participation has become a significant research frontier in both \lizhi{psychometrics} and computational linguistics~\cite{korukonda2007differences,chittaranjan2011s,gavrilescu2018predicting,cai2022identifying}.
Consequently, the search for an automatic, unbiased method to assess personality traits without direct client participation has emerged as a significant research frontier in both psychometrics and computational linguistics~\cite{korukonda2007differences,chittaranjan2011s,gavrilescu2018predicting,cai2022identifying}.

% \YY{TODO: There's a logical gap that why LLM is suitable for this task, directly point out the drawbacks and echo to capabilities of LLMs}

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=\linewidth]{figures/illustration_example.pdf}
%     \caption{Example of predicting BFI traits from counseling dialogues using LLMs. LLMs are conditioned by counseling dialogues and play the role of clients to fill in the BFI questionnaire and predict the BFI traits. ``Con'' indicates ``Conscientiousness'', ``Agr'' indicates ``Agreeableness'', and ``Neg Emot'' indicates ``Negative Emotionality''.}
%     \label{fig:illustration-mini}
% \end{figure}

\begin{figure*}[t]
    \centering
    \includegraphics[width=0.7\textwidth]{figures/illustration.pdf}
    \caption{Examples of predicting BFI traits from counseling dialogues using LLMs. LLMs are conditioned by counseling dialogues and play the role of clients to fill in the BFI questionnaire and predict the BFI traits. ``Con'' indicates ``Conscientiousness'', ``Agr'' indicates ``Agreeableness'', and ``Neg Emot'' indicates ``Negative Emotionality''.}
    \label{fig:illustration}
\end{figure*}

% \YY{Paragraph 3: What is my key idea in approaching this problem?}

Recent advancements in Large Language Models (LLMs)~\cite{brown2020GPT3,openai2023gpt4,bai2023qwen,geminiteam2024gemini} have revolutionized natural language processing (NLP), showcasing remarkable capabilities in text comprehension, reasoning, and role-playing.
% These advancements present an exciting opportunity to tackle the longstanding challenges of psychological assessment \lizhi{specify the challenges here, I guess you want to say something about subjective bias and time-consuming of self-report?}\YY{Actually, challenges come from poor performance of traditional NLP tools}.
These developments offer a promising opportunity to address the longstanding challenges of psychological assessment, particularly the issues of the time-consuming nature and subjective bias of self-report measures.
% \lizhi{To address the challenge in the field of psycho-counseling, we asked:} \textbf{Can LLMs predict personality traits based on counseling dialogues?} The question drives our investigation into the potential of LLMs to accurately predict the BFI traits from counseling dialogues, exploring both zero-shot and fine-tuning methodologies.
Thus, we pose the research question: \textbf{Can LLMs predict personality traits based on counseling dialogues?} This question drives our investigation into the potential of LLMs to accurately predict BFI traits from counseling dialogues, exploring both zero-shot and fine-tuning methodologies.

% \YY{Paragraph 4: important technical details}

To answer this, we leverage role-play and questionnaire-based approaches within LLMs as effective prompt engineering strategies.
% \lizhi{here refine to the plural form}.
Role-playing allows LLMs to simulate interactive dialogues, capturing the dynamic and context-sensitive aspects of human interactions~\cite{ng2024llms} essential for understanding complex personality traits.
% Conversely, the items of questionnaires measuring personality provide structured input and {\color{red} split a hard task into several easy ones} \lizhi{why you put words here into red?} that ensures alignment with established psychological constructs.  
Conversely, the items of questionnaires measuring personality provide structured input that divides and conquers the original and complex predicting task~\cite{john1991big,soto2017next}, ensuring alignment with established psychological constructs.
Combining these methods enhances the model's ability to generate nuanced responses and improves the effectiveness of personality predictions.

\input{tables/statistics_dialogues.tex}

In this context, we unfold our research in three stages.
% First, \lizhi{we evaluate the prompt strategies that questionnaire-based approaches and role-play scenarios to predict BFI personality traits}. 
First, we evaluate the effectiveness of prompt strategies using questionnaire-based approaches and role-play scenarios to predict BFI personality traits.
We then examine factors influencing prediction validity, including the roles of role-play, the types and scales of LLMs, and the granularity of counseling sessions.
Finally, we enhance LLM performance through fine-tuning with generated reasoning results, aiming to boost prediction efficacy and validity.

% \YY{Paragraph 5: How to evaluate the effectiveness of my method? and the most impressive results}

% To validate our approach of personality prediction, we conduct a comprehensive evaluation using 853 real-world counseling sessions, comparing the LLM-predicted BFI traits with ground-truth traits obtained from 83 clients. 
To evaluate our framework, we performed an extensive assessment that included 853 real-wrold counseling sessions, juxtaposing the BFI traits predicted by the LLM with the ground-truth traits obtained from 83 clients using Pearson correlation. Our findings indicate that the correlation is robust and significant.
% \lizhi{Furthermore}, a detailed error analysis by sessions and user illuminates the strengths and limitations of our method, offering invaluable insights for future research.
Additionally, an in-depth error analysis across models, sessions, and users highlights the strengths and weaknesses of our framework, providing crucial insights for future studies.

% \YY{Paragraph 6: Summary of key contributions}

% Our findings can be summarized as follows:

% % \YY{TODO: summarize the contributions into three points: 1. framework, 2. results, 3. error analysis}

% \noindent \textbf{1.} \textit{We propose a novel, automatic framework to effectively predict the BFI traits from counseling dialogues with Role-play and Questionnaire-based approaches using Large Language Models.} \\
% % Experiments of our framework, comfirming validity and reliability, finding that with only 40\% content of a counselling session, LLMs can already predict big five personality traits.\\
% \noindent \textbf{2.} \textit{We conduct a thorough investigation on validity, with 853 real-world counseling sessions, demonstrating a significant and strong correlation between the predict and groud-truth BFI traits, and LLMs can already predict BFI traits based on only 40\% content of a counselling session.} \\
% \noindent \textbf{3.} \textit{We further align the Llama3-8B model with the counseling dialogues by DPO fine-tuning, achieveing 130.95\% improvement in validity and beating the state-of-the-art of Qwen1.5-110B by 17.81\%. We release our code and model for future research.}

\input{tables/method_ablation.tex}

Our contributions are as follows:
\begin{enumerate}[leftmargin=0pt, itemindent=1em, itemsep=0pt, parsep=0pt]
    \item \textbf{Innovative Framework:} We propose a novel framework that combines role-play and questionnaire-based prompting within LLMs to predict BFI traits from counseling dialogues. This method effectively captures dynamic human interactions and aligns with established psychological constructs.
    \item \textbf{Empirical Validation:} Through extensive evaluation on 853 real-world counseling sessions, we demonstrate a strong correlation between LLM predictions and client-derived BFI traits, even with only 40\% of the session content. This provides robust empirical support for the accuracy of our framework.
    \item \textbf{Comprehensive Ablation Study:} We conduct a thorough ablation study to evaluate the impact of role-play and questionnaire strategies, types of 20 cutting-edge LLMs and scales from 7B to 110B, and session content granularity from 10\% to 100\% on prediction validity. The proposed framework superpass the different baselines in each ablation setting, demonstrating the effectiveness of our approach and ensuring generalizability. Our findings highlight the effectiveness of our framework in reducing self-awareness and social desirability biases.
    \item \textbf{Enhanced Effectiveness:} By fine-tuning the Llama3-8B model using DPO, we achieve a 130.95\% improvement in prediction validity, surpassing the state-of-the-art Qwen1.5-110B model by 17.81\%. This fine-tuning approach significantly enhances both the effectiveness and efficiency of the model, making our framework accessibility for more researcher. We release our code, model, and detailed instruction at \url{https://github.com/XXX/XXX} for future research, supporting reproducibility and further exploration.
\end{enumerate}

% \noindent \textbf{1.} \textit{We propose a novel, \lizhi{automatic method to predict the big five personality traits based on} counseling dialogues using Large Language Models.} \YY{TODO:``Method''->``Framework''}\\
% \noindent \textbf{2.} \textit{We conduct a thorough investigation using 853 counseling dialogues, demonstrating a significant correlation between the BFI traits predicted by LLMs and those derived from clients.} \\
% \noindent \textbf{3.} \textit{We perform a detailed error analysis, demonstrating the strengths and limitations of our approach, which will guide future research in this field.}

% \lizhi{the second and the third contribution need to be changed to the detail content of contribution instead of the description now. for examples, for the second one, you could say: we found the LLMs can already predict big five personality traits based on only 40\% content of a counselling session.}

% \YY{Roger that, TODO: polish the contributions with detailed content}

% \YY{Paragraph 7: Outline of the paper}






% \section{Introduction}
% \label{sec:intro}

% % % Background
% % Knowing an client's personality traits is crucial for providing effective psychological counseling~\cite{gordon2002said,anestis2021personality}.
% % % Counselors can use this information to tailor their advice and support to the client's needs, thereby improving the quality of counseling services~\cite{gavrilescu2018predicting,yeye2020predicting}. However, Personality, with its intricate complexity, presents significant obstacles to traditional methods of modeling and measurement. Established tools such as the Big Five Inventory, which is based on Item Response Theory~\cite{baker2001basics,reise2009item,embretson2013item}, require clients to provide direct answers to evaluate traits~\cite{chernyshenko2001fitting,khorramdel2014measuring}. 
% % % % However, the intrusive nature of these tools limits their usefulness in sensitive settings like psychological counseling.

% % This knowledge allows counselors to personalize their advice and support, thereby enhancing the overall quality of counseling services~\cite{gavrilescu2018predicting,yeye2020predicting}. However, the complexity of personality traits presents significant challenges for conventional modeling and measurement methods. Traditional tools such as the Big Five Inventory, which rely on Item Response Theory~\cite{baker2001basics,reise2009item,embretson2013item}, require clients to answer a series of questions, wchich is time-consuming and potentially leads to issues like subjective bias or social desirability bias, thereby compromising accuracy~\cite{chernyshenko2001fitting,khorramdel2014measuring,mccrae2007observer}. How to assess personality traits without direct client participation is a significant problem in the field of psychology and computational linguistics~\cite{korukonda2007differences,chittaranjan2011s,gavrilescu2018predicting,cai2022identifying}.

% \YY{Paragraph 1 \& 2: Why is the problem important? Why is the problem difficult?}

% % Understanding a client's personality traits is crucial for providing effective psychological counseling. Personalized advice based on these traits can significantly enhance the quality of counseling services~\cite{gordon2002said,anestis2021personality}.
% % % However, traditional methods for assessing personality traits following Item Response Theory~\cite{baker2001basics,reise2009item,embretson2013item}, such as the Big Five Inventory (BFI)~\cite{john1991big}, require clients to answer extensive questionnaires. This approach is requiring clients' participation and time-consuming, potentially leading to subjective bias and social desirability bias, compromising the accuracy of the assessment~\cite{chernyshenko2001fitting,khorramdel2014measuring,mccrae2007observer}.
% % However, the complexity of personality traits presents significant challenges for conventional modeling and measurement methods. Traditional tools like the Big Five Inventory (BFI)~\cite{john1991big}, which rely on Item Response Theory~\cite{baker2001basics,reise2009item,embretson2013item}, require clients to answer a series of questions, which is time-consuming and may lead to subjective bias or social desirability bias, compromising accuracy~\cite{chernyshenko2001fitting,khorramdel2014measuring,mccrae2007observer}. Automatically assessing personality traits without direct client participation remains a significant challenge in psychology and computational linguistics~\cite{korukonda2007differences,chittaranjan2011s,gavrilescu2018predicting,cai2022identifying}.

% Understanding a client's personality traits is paramount for effective psychological counseling. Personalized advice tailored to these traits can significantly enhance the quality of counseling services~\cite{gordon2002said,anestis2021personality}. Despite its importance, accurately assessing personality traits remains fraught with challenges. Traditional tools like the Big Five Inventory (BFI)~\cite{john1991big}, grounded in Item Response Theory~\cite{baker2001basics,reise2009item,embretson2013item}, necessitate clients to complete extensive questionnaires. This process is not only time-consuming but also susceptible to subjective biases and social desirability effects, undermining accuracy~\cite{chernyshenko2001fitting,khorramdel2014measuring,mccrae2007observer}. Consequently, the quest for an automatic, unbiased method to assess personality traits without direct client participation has become a significant research frontier in both psychology and computational linguistics~\cite{korukonda2007differences,chittaranjan2011s,gavrilescu2018predicting,cai2022identifying}.

% % Established tools relying on direct client participation are not only intrusive but also prone to biases, making them less effective in sensitive settings like psychological counseling. Moreover, the need for a non-intrusive, efficient, and accurate method for assessing personality traits remains a critical problem in both psychology and computational linguistics~\cite{korukonda2007differences,chittaranjan2011s,cai2022identifying}.

% % % challenge and why it is important
% % % The challenge of effectively assessing individuals' personality traits in a non-intrusive way is a key issue in psychology~\cite{korukonda2007differences,chittaranjan2011s,gavrilescu2018predicting,cai2022identifying}. Our practical experience and related researches~\cite{gordon2002said,anestis2021personality} suggest that understanding an individual's personality in counseling sessions is crucial as it allows for personalized support and advice, providing valuable insights into their mental well-being and thereby improving the quality of counseling services~\cite{gavrilescu2018predicting,yeye2020predicting}. Yet, predicting the Big Five traits in counseling sessions is a challenging task due to the complexity of these traits and the limitations of traditional assessment methods.
% % % 在心理咨询场景(~\ref{appendix:jargon:scene})中，\textbf{了解来访者的人格特质(~\ref{appendix:jargon:trait})对于提升咨询服务的质量和效果至关重要。}目前，人格特质的评估主要依赖于让来访者完成自评问卷。自评问卷(~\ref{appendix:jargon:self-assessment})是个体回答有关自己思维、感受和行为的问题；以大五人格为例，大五人格问卷（BFI）是目前信度、效度稳定且业内运用最广泛的在人格评估方法，衡量了个体在开放性、尽责性、外向性、宜人性和神经质五个方面的人格特质~\cite{zhang2022big}。一般情况下，来访者会在咨询开始前对问卷量表进行填写,但自评量表存在耗时、有主观偏差、社会期望偏差(~\ref{appendix:jargon:bias})等问题，可能对后续心理咨询造成不利影响。因此，需要一种相对客观、高效、准确的人格特征评估方法，以帮助提高心理咨询服务的效率。
% % % The difficulty in assessing personality traits without direct client participation poses a significant problem in the field of psychology and computational linguistics~\cite{korukonda2007differences,chittaranjan2011s,gavrilescu2018predicting,cai2022identifying}. 
% % \YY{TODO: logical conflicts here, explain what are the challenges and why it is important.}
% % % Understanding a client's personality traits during counseling sessions is crucial, as it provides valuable insights into their mental well-being and allows for tailored support~\cite{gavrilescu2018predicting,yeye2020predicting}. 

% % % However, predicting the Big Five traits in counseling sessions is inherently complex due to the multifaceted nature of these traits and the limitations of traditional assessment methods.

% % % Previous work
% % % Previous studies have explored the prediction of the Big Five personality traits using various methods, such as self-report, observer rating~\cite{mihura2003correspondence,mccrae2007observer,gamble2024understanding}, linguistic analysis~\cite{yeye2020predicting,koutsoumpis2022kernel}, and machine learning algorithms~\cite{gavrilescu2018predicting,abe2020big}. However, these approaches face challenges in terms of effectiveness, interpretability, and model capability.
% % % For example, external human observers could use expert knowledge to extract personality traits from conversations, but always suffer from low-efficiency and sometimes subjective judgments~\cite{mccrae2007observer}. Linguistic analyses offer valuable insights, but may not fully capture the intricacies of personality expression~\cite{koutsoumpis2022kernel}. Data-driven techniques like machine learning show promise but require extensive annotated data and is limited by model's capability~\cite{abe2020big}, including length of text window, multi-lingual support, and the ability to generate human-like responses.

% % % 针对上述问题，出现了许多针对性的解决方法。其中，他评问卷(~\ref{appendix:jargon:other-assessment})是由心理学家或训练有素的观察者根据个体在特定情况下的行为来评估其人格，能够实现独立、无需来访者参与的人格评估，能够有效解决自评问卷所带来的主观偏差与社会期望偏差等问题；通过语言分析从心理咨询对话记录中提取关键词、句式等语言特征，能够自动化地分析来访者的人格特质，提高了评估的效率；在心理学的其他领域研究，如基于社交媒体数据的人工预测，出现了通过机器学习模型预测人格特征的方法，通过以数据驱动的方法，从大量数据中学习到来访者的人格特征，提升了预测的准确性和可靠性。但是，这些方法仅解决了目前人格评估方法的一部分问题，仍然存在着预测准确性、效率、和可解释性(\ref{appendix:jargon:interpretability})上的不足。

% % Previous studies have explored predicting personality traits without direct client participation using various methods, such as observer ratings~\cite{mihura2003correspondence,mccrae2007observer,gamble2024understanding}, linguistic analysis~\cite{yeye2020predicting,koutsoumpis2022kernel}, and machine learning algorithms~\cite{gavrilescu2018predicting,abe2020big}. However, these approaches face challenges in terms of effectiveness, interpretability, and model capability. For example, external human observers could use expert knowledge to extract personality traits from conversations, but always suffer from low-efficiency and sometimes subjective judgments~\cite{mccrae2007observer}. Linguistic analyses offer valuable insights, but may not fully capture the intricacies of personality expression~\cite{koutsoumpis2022kernel}. Data-driven techniques like machine learning show promise but require extensive annotated data and are limited by model capability~\cite{abe2020big}, including the length of the text window, multi-lingual support, and the explainability of the model.

% % % Various studies have explored different methods for predicting the Big Five personality traits, including self-reporting, observer ratings~\cite{mihura2003correspondence,mccrae2007observer,gamble2024understanding}, linguistic analysis~\cite{yeye2020predicting,koutsoumpis2022kernel}, and machine learning algorithms~\cite{gavrilescu2018predicting,abe2020big}. Yet these approaches have their own limitations. Observer ratings, while leveraging expert knowledge, often suffer from inefficiency and subjective judgments~\cite{mccrae2007observer}. Linguistic analysis, though valuable, may not capture all nuances of personality expression~\cite{koutsoumpis2022kernel}. Machine learning algorithms, while promising, require extensive annotated data and face constraints related to model capacity, such as text window length and multilingual support~\cite{abe2020big}.

% \begin{figure*}[t]
%     \centering
%     \includegraphics[width=0.8\textwidth]{example-image-golden}
%     \caption{Illustration of our method. To be replaced}
%     \label{fig:illustration}
% \end{figure*}

% \YY{Paragraph 3: What is my key idea in approaching this problem?}

% % % Our approach
% % % Given the constraints of current methods and the evolving capabilities of Large Language Models (LLMs) in processing and generating text that resembles human language, we introduce a pioneering strategy. Our approach utilises the "role-play" capability of LLMs to predict the Big Five personality traits from counseling conversations. By employing LLMs to imitate a client in counseling sessions based on their dialogues and then undertaking the client, we can directly model and evaluate individuals' personality traits. This novel approach distinguishes itself from prior studies by providing a direct evaluation pathway, thus aligning more closely with the Item Response Theory. The integration of LLMs in this scenario not only avoids the intrusive nature of traditional approaches, but also offers scalability and detailed capture of personality nuances within conversations. As a result, this method is positioned to provide accurate forecasts of the Big Five personality traits, offering insights into individuals' psychological states, and making substantial contributions to the enhancement of counseling services and a deeper understanding of human behaviour.
% % % Inspired by evolving capability of Large Language Models (LLMs)~\cite{brown2020GPT3,openai2023gpt4,bai2023qwen,geminiteam2024gemini}, which show promise in complex text understanding, reasoning, generation, and role-play, it comes a natural question: \textbf{Can we leverage LLMs to predict the Big Five personality traits from counseling dialogues?} To address this question, we test several settings and find that LLMs can predict the Big Five personality traits with high accuracy, reliability, and validity by playing client of counseling dialogues to fill the questionnaire of client. Our findings suggest that LLMs can be a powerful tool for non-intrusive personality assessment in counseling sessions, offering valuable insights into individuals' psychological states and enhancing the quality of counseling services.

% % % Given the evolving capabilities of Large Language Models (LLMs)~\cite{brown2020GPT3,openai2023gpt4,bai2023qwen,geminiteam2024gemini}, which demonstrate advanced text comprehension, reasoning, generation, and role-play, we ask a pivotal question: \textbf{Can LLMs be leveraged to predict the Big Five personality traits from counseling dialogues?} To answer this, we explored various settings and discovered that LLMs could predict the Big Five traits with high accuracy, reliability, and validity by simulating the client in counseling dialogues and filling out personality questionnaires.

% % Recent development in Large Language Models (LLMs)~\cite{brown2020GPT3,openai2023gpt4,bai2023qwen,geminiteam2024gemini} demonstrates advanced ability in text comprehension, reasoning, as well as role-play, and also the potential in Psychology. With this we ask a pivotal research question: \textbf{Can LLMs predict the personality traits based on counseling dialogues?} 
% % % To answer this, we try to leverage LLM in prompt-level as well as in fine-tuning level to extract personality information from dialogues and spliting the challenge task of immediately prediction into several sub-tasks of filling the questionnaire.
% % To answer this, we systematically investigate the effectiveness of LLMs in predicting the Big Five personality traits from counseling dialogues with zero-shot and fine-tuning settings.
% % % Our approach leverages the "role-play" capability of LLMs to simulate a client in counseling sessions, thereby predicting personality traits without direct client participation. This innovative method aligns more closely with the principles of Item Response Theory while avoiding the intrusive nature of traditional approaches.
% In recent years, the advent of Large Language Models (LLMs)~\cite{brown2020GPT3,openai2023gpt4,bai2023qwen,geminiteam2024gemini} has revolutionized natural language processing, demonstrating remarkable capabilities in text comprehension, reasoning, and even role-playing. These advancements present an exciting opportunity to tackle the longstanding challenges of psychological assessment. Our pivotal research question emerges: \textbf{Can LLMs predict personality traits based on counseling dialogues?} This question drives our investigation into the potential of LLMs to accurately predict the Big Five personality traits from counseling dialogues, exploring both zero-shot and fine-tuning methodologies.

% \YY{Paragraph 4: important technical details}
% % % % To assess the efficiency of our method, we carry an extensive investigation using 853 psychological counseling sessions gathered from our platform. We perform role-play of client, as well as counselor and observer, to gain a thorough insight into the Big Five personality characteristics in counseling discussions with various cutting-edge LLMs, such as Qwen1/1.5~\cite{bai2023qwen}, Yi~\cite{ai2024yi}, AquilaChat2~\cite{Aquila2}, Baichuan2~\cite{bai2023qwen}, Gemma~\cite{gemmateam2024gemma}, and ChatGLM3~\cite{zeng2023glmb}.
% % % % % GPT-4, and Gemini-Ultra. 
% % % % Our findings indicate a notable connection between the Big Five personality traits anticipated by LLMs and those derived from clients. Additionally, we conducted a meticulous error assessment to pinpoint the advantages and constraints of our methodology.
% % % To validate our method's effectiveness, we conducted a comprehensive study using 853 psychological counseling sessions from our platform. We utilized role-play scenarios, where LLMs assumed the roles of clients, counselors, and observers, to assess the Big Five personality traits with several settings of cutting-edge LLMs, different granularity, and model sizes.
% % % % , including Qwen 1/1.5~\cite{bai2023qwen}, Yi~\cite{ai2024yi}, AquilaChat2~\cite{Aquila2}, Baichuan2~\cite{bai2023qwen}, Gemma~\cite{gemmateam2024gemma}, and ChatGLM3~\cite{zeng2023glmb}.
% % % Our findings demonstrate a strong and significant correlation between the Big Five traits predicted by LLMs and those derived from direct client participation. Additionally, we performed a detailed error analysis to present the strengths and limitations of our methodology.

% % We first investigate the way of predicting the BFI traits, including w/ and w/o questionnaire and role-play. \YY{TODO: polish it.} We then investigate the factors that may affect the prediction of BFI traits, including the role of the role-play, the type, and scale of LLMs, and the granularity of counseling sessions. We finally fine-tuning the LLMs with the generated reasoning results to improve the prediction accuracy.

% To answer this, we leverage role-play and questionnaire-based approaches within LLMs as an effective prompt engineering strategy. Role-playing enables LLMs to simulate interactive dialogues, capturing the dynamic and context-sensitive aspects of human interactions essential for understanding complex traits. Conversely, questionnaires provide structured input and split a hard task into several easy ones that ensures alignment with established psychological constructs. Combining these methods enhances the model's ability to generate nuanced responses and improves the robustness and reliability of trait predictions.

% Our research unfolds in several stages. First, we explore methods for predicting BFI traits, evaluating both questionnaire-based approaches and role-play scenarios. We then scrutinize factors influencing prediction accuracy, including the role of role-play, the type and scale of LLMs, and the granularity of counseling sessions. Finally, we enhance LLM performance through fine-tuning with generated reasoning results, aiming to boost prediction accuracy.

% \YY{Paragraph 5: How to evaluate the effectiveness of my method? and the most impressive results}

% To validate our approach, we conduct a comprehensive evaluation using 853 real-world counseling sessions, comparing the LLM-predicted BFI traits with ground-truth traits obtained from 83 clients. Our analysis reveals a robust correlation between the LLM predictions and direct client-derived traits. Additionally, a detailed error analysis by session and user illuminates the strengths and limitations of our method, offering invaluable insights for future research.

% \YY{Paragraph 6: Summary of key contributions}



% Our findings can be summarized as follows:
% % % \begin{itemize}
% % %   \item We present an novel non-disruptive method for predicting the Big Five personality traits from counseling dialogues by employing LLMs.
% % %   \item We carry out an extensive investigation to assess the efficiency of our method using 853 counseling dialogues and reveal a notable connection between the Big Five personality traits anticipated by LLMs and those derived from individuals.
% % %   \item We undertake a thorough examination of errors to recognize the advantages and constraints of our method, offering valuable insights for future studies in this field.
% % % \end{itemize}

% % \noindent \textbf{1.} \textit{We present a novel non-intrusive method for predicting the Big Five personality traits from counseling dialogues by employing LLMs.}\\
% % \noindent \textbf{2.} \textit{We carry out an extensive investigation to assess the efficiency of our method using 853 counseling dialogues and reveal a notable connection between the Big Five personality traits anticipated by LLMs and those derived from individuals.}\\
% % \noindent \textbf{3.} \textit{We undertake a thorough examination of errors to recognize the advantages and constraints of our method, offering valuable insights for future studies in this field.}

% \noindent \textbf{1.} \textit{We propose a novel, participation-free method for predicting the Big Five traits from counseling dialogues using Large Language Models.} \\
% \noindent \textbf{2.} \textit{We conduct a thorough investigation using 853 counseling dialogues, demonstrating a significant correlation between the Big Five traits predicted by LLMs and those derived from clients.} \\
% \noindent \textbf{3.} \textit{We perform a detailed error analysis, demonstrating the strengths and limitations of our approach, which will guide future research in this field.}

% \YY{Paragraph 7: Outline of the paper}


==> sec/2.related_works.tex <==
\section{Related Work}

% In exploring the automated measurement of the BFI traits using LLMs in counseling dialogues, we draw upon advancements in both automatic personality assessment and the application of LLMs in psychological contexts.

% Not a mere description of the state-of-the art.
% Serves two purposes:
% § show you know the state-of-the-art;
% § show your method solves
% – aspects of the problem that were not solved before, or
% – a new problem.

% \subsection{Automatic Personality Assessment in Counseling}

\paragraph{Automatic Assessment}


% \YY{Previous works on automatic personality assessment}
% % The automatic assessment of personality traits has been a subject of extensive research, with studies focusing on leveraging machine learning and natural language processing techniques to predict the BFI traits from text data. 
% % \citet{sun2018personality} were among the first to utilize text structure, employing a bidirectional LSTM with CNN and Latent Sentence Groups to abstract features from text. This approach demonstrated the significance of text structure in personality analysis. Extending this, \citet{mehta2020bottom} combined psycholinguistic features with language model embeddings, setting a new benchmark in personality prediction and providing insights into feature influence. The effectiveness of ensemble models was highlighted by \citet{Christian2021TextBP}, who integrated BERT~\cite{devlin2019bert}, RoBERTa~\cite{liu2019roberta}, and XLNet~\cite{yang2019xlnet} to enhance trait prediction from social media. \citet{ramezani2022text} introduced a novel use of knowledge graph attention networks in their KGrAt-Net, improving prediction accuracies by simulating cognitive semantic understanding. Further, \citet{zhu2022perkg} incorporated psycholinguistic knowledge into a personality knowledge graph, addressing data scarcity and demonstrating the value of external knowledge bases. The latest work by \citet{johnson2023aspect} employed an aspect-aware psycholinguistic knowledge graph, enhancing deep learning models with ontology and emotion lexicons for refined personality trait detection.

% % Previous works on automatic personality assessment have extensively employed natural language processing techniques to predict the BFI traits from text data.
% The automatic assessment of personality traits has been a subject of extensive research, with studies focusing on leveraging machine learning and natural language processing techniques to predict the BFI traits from text data.
% % \citet{sun2018personality} used a bidirectional LSTM and CNN to highlight the importance of text structure in personality analysis.
% \citet{sun2018personality} employed a bidirectional LSTM and CNN to predict personality traits from text data, demonstrating the significance of text structure in personality analysis.
% % \citet{mehta2020bottom} set new benchmarks by combining psycholinguistic features with language model embeddings.
% \citet{mehta2020bottom} replaced hand-crafted features with language model embeddings, and achieved performance improvements in personality prediction.
% These two works suggest the effectiveness of text structure and feature engineering in personality analysis with machine learning models.
% % \citet{Christian2021TextBP} demonstrated the effectiveness of language models by integrating BERT, RoBERTa, and XLNet for enhanced trait prediction.
% \citet{Christian2021TextBP} reported with the integration of pre-trained language models, such as BERT, RoBERTa, and XLNet, the performance of personality prediction models can be significantly improved.
% % \citet{ramezani2022text} improved prediction accuracies using knowledge graph attention networks in KGrAt-Net, simulating cognitive semantic understanding.
% % \citet{zhu2022perkg} tackled data scarcity by incorporating psycholinguistic knowledge into a personality knowledge graph.
% % \citet{johnson2023aspect} further refined trait detection by enhancing deep learning models with an aspect-aware psycholinguistic knowledge graph.
% \YY{These graph-based tricks make non-sense here, TODO: add more works, e.g. MBTI prediction using LLMs here.}
% These works show promise in employing natural language processing techniques for automatic personality assessment, but limited by capability of traditional NLP tools and method, there's no work using LLMs to predict BFI traits in counseling dialogues.
% % \lizhi{are there any differences between the above mentioned works and our current work? use a sentence to specify the differences.}

The automatic assessment of personality traits has been widely studied, with numerous works using machine learning or NLP techniques to predict BFI traits from textual data. \citet{sun2018personality} were trailblazers in employing a bidirectional LSTM combined with CNN to predict personality traits, highlighting the importance of text structure. Building on this, \citet{mehta2020bottom} showed that substituting hand-crafted features with language model embeddings enhanced the accuracy of personality prediction. These studies highlight the efficacy of text structure and feature engineering in personality analysis using machine learning models. \citet{Christian2021TextBP} further progressed this domain by incorporating pre-trained language models, demonstrating improvements in predicting personality traits.

Despite these advancements, traditional NLP techniques have limitations in fully capturing the nuances of personality traits from text data. To date, no studies have used LLMs to predict BFI traits in counseling dialogues, leaving a significant gap in the literature.

\input{tables/role_ablation.tex}


% \subsection{Application of LLMs in Psychology}

\paragraph{Application of LLMs in Psychology}

% \YY{Previous works on applying LLMs in psychology}

% % LLMs have seen extensive development and success, with models like GPT-3/4~\cite{brown2020GPT3,openai2023gpt4}, PaLM~\cite{anil2023palm}, and others like Llama2~\cite{touvron2023llama}, QWen~\cite{bai2023qwen} being applied across various fields, including psychology~\cite{demszky2023using}. \citet{li2022automated} demonstrated the potential of LLMs in evaluating text-based counseling interactions, emphasizing the challenges in data collection within sensitive domains. \citet{fu2023enhancing}'s decision-support system for psychological counseling showcases LLMs' ability to aid non-professionals. \citet{wang2023emotional}'s study on emotional intelligence (EI) found that GPT-4 exhibited high EI levels, providing insights into LLMs' emotional processing capabilities. In a novel approach, \citet{pellert2023ai} applied psychometric inventories to LLMs, suggesting the inadvertent acquisition of human-like traits. \citet{blancocuaresma2024psychological} proposed a privacy-centric method for psychological assessment, focusing on cost-effective and privacy-sensitive applications. Lastly, \citet{xu2024mentalllm} evaluated LLMs for mental health prediction, noting the importance of instruction fine-tuning and the ethical considerations in real-world applications.

% Though LLMs have not been used automatically for personality assessment in counseling so far, they have been widely applied in psychology for various tasks, including text-based counseling, emotional intelligence evaluation, and mental health prediction.

% \YY{Feasibility}
% % Automated real-time evaluation of counselor-client interaction is important for ensuring quality counseling but the rules are difficult to articulate. Recent advancements in machine learning methods show the possibility of learning such rules automatically. However, these methods often demand large scale and high quality counseling data, which are difficult to collect. To address this issue, we build an online counseling platform, which allows professional psychotherapists to provide free counseling services to those are in need. In exchange, we collect the counseling transcripts. Within a year of its operation, we manage to get one of the largest set of (675) transcripts of counseling sessions. To further leverage the valuable data we have, we label our dataset using both coarse- and fine-grained labels and use a set of pretraining techniques. In the end, we are able to achieve practically useful validity in both labeling system.
% Many recent works have demonstrated the feasibility of using LLMs to extract personality traits.
% \citet{li2022automated} demonstrated the potential of LLMs in evaluating text-based counseling interactions, emphasizing the challenges in data collection within sensitive domains.
% % Large Language Models (LLMs) have demonstrated remarkable abilities across numerous disciplines, primarily assessed through tasks in language generation, knowledge utilization, and complex reasoning. However, their alignment with human emotions and values, which is critical for real-world applications, has not been systematically evaluated. Here, we assessed LLMs' Emotional Intelligence (EI), encompassing emotion recognition, interpretation, and understanding, which is necessary for effective communication and social interactions. Specifically, we first developed a novel psychometric assessment focusing on Emotion Understanding (EU), a core component of EI, suitable for both humans and LLMs. This test requires evaluating complex emotions (e.g., surprised, joyful, puzzled, proud) in realistic scenarios (e.g., despite feeling underperformed, John surprisingly achieved a top score). With a reference frame constructed from over 500 adults, we tested a variety of mainstream LLMs. Most achieved above-average EQ scores, with GPT-4 exceeding 89% of human participants with an EQ of 117. Interestingly, a multivariate pattern analysis revealed that some LLMs apparently did not reply on the human-like mechanism to achieve human-level performance, as their representational patterns were qualitatively distinct from humans. In addition, we discussed the impact of factors such as model size, training method, and architecture on LLMs' EQ. In summary, our study presents one of the first psychometric evaluations of the human-like characteristics of LLMs, which may shed light on the future development of LLMs aiming for both high intellectual and emotional intelligence. 
% \citet{wang2023emotional} evaluated GPT-4's emotional intelligence, providing insights into LLMs' emotional processing capabilities.
% % Despite the many use cases for large language models (LLMs) in creating personalized chatbots, there has been limited research on evaluating the extent to which the behaviors of personalized LLMs accurately and consistently reflect specific personality traits. We consider studying the behavior of LLM-based agents which we refer to as LLM personas and present a case study with GPT-3.5 and GPT-4 to investigate whether LLMs can generate content that aligns with their assigned personality profiles. To this end, we simulate distinct LLM personas based on the Big Five personality model, have them complete the 44-item Big Five Inventory (BFI) personality test and a story writing task, and then assess their essays with automatic and human evaluations. Results show that LLM personas' self-reported BFI scores are consistent with their designated personality types, with large effect sizes observed across five traits. Additionally, LLM personas' writings have emerging representative linguistic patterns for personality traits when compared with a human writing corpus. Furthermore, human evaluation shows that humans can perceive some personality traits with an accuracy of up to 80%. Interestingly, the accuracy drops significantly when the annotators were informed of AI authorship.
% \citet{jiang2024personallm} proposed to study personalized LLM personas with coherence between their generated story and BFI traits and found that LLM personas' self-reported BFI scores are consistent with their designated personality types.

LLMs have undergone significant advances in numerous fields, including psychology.
Notable models such as GPT-3 and GPT-4~\cite{brown2020GPT3,openai2023gpt4}, Llama2~\cite{touvron2023llama}, and QWen~\cite{bai2023qwen} have been applied in psychological contexts with promising results.
\citet{li2022automated,li2023understanding} demonstrated the potential of LLM in evaluating text-based counseling interactions, highlighting the challenges inherent in data collection within sensitive domains.
\citet{wang2023emotional} evaluated GPT-4's emotional intelligence, providing insight into LLM's emotional processing capabilities.
Furthermore, \citet{jiang2024personallm} investigated the alignment between the content produced by LLMs and their assigned personality profiles, finding that the self-reported BFI scores are consistent with their attributed personality types.

% \YY{MBTI}
% Myers Briggs Type Indicator (MBTI)~\cite{myers1962myers} tests has been invloved in the evaluation of LLMs' personality traits in various works for its easy-to-understand and widely-used nature.
% \citet{pan2023llms} and \citet{huang2023chatgpt} investigate the feasibility of MBTI to evaluate LLMs' personality types, and show the potential of employing Psychological Tools in LLMs' evaluation.
% % Large Language Models (LLMs) especially ChatGPT have produced impressive results in various areas, but their potential human-like psychology is still largely unexplored. Existing works study the virtual personalities of LLMs but rarely explore the possibility of analyzing human personalities via LLMs. This paper presents a generic evaluation framework for LLMs to assess human personalities based on Myers Briggs Type Indicator (MBTI) tests. Specifically, we first devise unbiased prompts by randomly permuting options in MBTI questions and adopt the average testing result to encourage more impartial answer generation. Then, we propose to replace the subject in question statements to enable flexible queries and assessments on different subjects from LLMs. Finally, we re-formulate the question instructions in a manner of correctness evaluation to facilitate LLMs to generate clearer responses. The proposed framework enables LLMs to flexibly assess personalities of different groups of people. We further propose three evaluation metrics to measure the consistency, robustness, and fairness of assessment results from state-of-the-art LLMs including ChatGPT and GPT-4. Our experiments reveal ChatGPT's ability to assess human personalities, and the average results demonstrate that it can achieve more consistent and fairer assessments in spite of lower robustness against prompt biases compared with InstructGPT.
% \citet{rao2023can} proposed to generate unbiasd prompts for LLMs to assess human personalities based on MBTI tests.

% Myers-Briggs Type Indicator (MBTI) tests~\cite{myers1962myers} have also been used to evaluate LLMs' personality traits due to their straightforward and widely-used nature.
Recent works have explored the use of Myers-Briggs Type Indicator (MBTI) tests~\cite{myers1962myers} to evaluate LLM personality traits due to their straightforward and widely used nature.
Studies by \citet{pan2023llms} and \citet{huang2023chatgpt} have investigated the feasibility of using MBTI to assess the personality types of LLMs, demonstrating the potential for the use of psychological tools in the evaluation of LLM.
Moreover, \citet{rao2023can} proposed generating unbiased prompts for ChatGPT to assess human personalities based on MBTI tests, further illustrating the integration of psychological tests with LLM.

% \YY{Role-play and Prompt Engineering}
% Role-play enables LLM to interact in a more human-like manner, brings more potential in Psychology.
% % Role-playing agents (RPAs), powered by large language models, have emerged as a flourishing field of applications. However, a key challenge lies in assessing whether RPAs accurately reproduce the personas of target characters, namely their character fidelity. Existing methods mainly focus on the knowledge and linguistic patterns of characters. This paper, instead, introduces a novel perspective to evaluate the personality fidelity of RPAs with psychological scales. Overcoming drawbacks of previous self-report assessments on RPAs, we propose InCharacter, namely Interviewing Character agents for personality tests. Experiments include various types of RPAs and LLMs, covering 32 distinct characters on 14 widely used psychological scales. The results validate the effectiveness of InCharacter in measuring RPA personalities. Then, with InCharacter, we show that state-of-the-art RPAs exhibit personalities highly aligned with the human-perceived personalities of the characters, achieving an accuracy up to 80.7%.
% \citet{wang2024incharacter} employed LLMs to evaluate the personality fidelity of Role-playing agents with several metrics, including psychological scales, and achieved an accuracy up to 80.7\%.
% % Modern large language models (LLMs) exhibit a remarkable capacity for role-playing, enabling them to embody not only human characters but also non-human entities. This versatility allows them to simulate complex human-like interactions and behaviors within various contexts, as well as to emulate specific objects or systems. While these capabilities have enhanced user engagement and introduced novel modes of interaction, the influence of role-playing on LLMs' reasoning abilities remains underexplored. In this study, we introduce a strategically designed role-play prompting methodology and assess its performance under the zero-shot setting across twelve diverse reasoning benchmarks. Our empirical results illustrate that role-play prompting consistently surpasses the standard zero-shot approach across most datasets. Notably, in experiments conducted using ChatGPT, accuracy on AQuA rises from 53.5% to 63.8%, and on Last Letter from 23.8% to 84.2%.Upon further comparison with the Zero-Shot-CoT technique, which prompts the model to "think step by step", our study demonstrates that role-play prompting acts as a more effective trigger for the CoT process. This highlights its potential to augment the reasoning capabilities of LLMs. 
% \citet{kong2024better} extend the role-play prompting methodology to assess its performance under the zero-shot setting across twelve diverse reasoning benchmarks.

% % \citet{fu2023enhancing} developed a decision-support system for psychological counseling, showcasing LLMs' ability to aid non-professionals.

% % \citet{pellert2023ai} applied psychometric inventories to LLMs, suggesting the inadvertent acquisition of human-like traits.
% % \citet{blancocuaresma2024psychological} proposed a privacy-centric method for psychological assessment, focusing on cost-effective and privacy-sensitive applications.
% % Lastly, \citet{xu2024mentalllm} evaluated LLMs for mental health prediction, noting the importance of instruction fine-tuning and ethical considerations in real-world applications.

Role-play techniques have enabled LLMs to interact in a more human-like manner, enhancing their application in psychology.
\citet{wang2024incharacter} used LLM-powered role-playing agents to evaluate the fidelity of character personality with scales.
\citet{kong2024better} extended role-play prompting methodologies to assess performance in various reasoning benchmarks, demonstrating improvements.
% \YY{Also mention some tech used in this paper, prompt engineering, role-play, DPO fine-tuning, offering context why we use them}
% \lizhi{again, specify the detail content of the above mentioned research, the detail content I mean what elements of decision making system aid non-human professionals and in what kind of way; also, how these research relates with our work?}

% Together, these works highlight the expanding role of LLMs in psychological assessment, while also acknowledging the challenges related to data privacy, ethics, and the accurate emulation of human emotional intelligence \lizhi{I don't get why "the accurate emulation of human emotional intelligence" appears here}.
These studies underscore the growing role of LLMs in psychological assessment. Our research builds on this by using LLMs to predict BFI traits from counseling dialogues, employing techniques like prompt engineering and role-play to enhance prediction effectiveness.



==> sec/3.method.tex <==
\section{Framework for Predicting BFI Traits}

% % \YY{For psychological contributions, we propose a novel, participation-free framework for predicting the BFI traits from counseling dialogues using Large Language Models. Repalce original "method" with "Framework of ..."}

% In this study, we propose a novel framework for predicting the personality traits from counseling dialogues using LLMS. Our framework encompasses prompt design, LLM conditioning, and the evaluation metrics essential for gauging the efficacy of our approach.

% % % This section delineates the methodology employed for leveraging LLMs to infer the BFI traits from counseling dialogues. Our approach encompasses data collection and preprocessing, LLM conditioning for personality trait prediction, a novel role-play strategy for simulating counseling scenarios, and the evaluation metrics adopted to gauge the efficacy of our method.

% % This section delineates the methodology used to leverage LLMs to infer the BFI traits from counseling dialogues. It includes data collection and preprocessing, conditioning LLMs for personality trait prediction, and evaluating the method's efficacy through validity and reliability metrics.

This section presents our framework, which consists of three main elements: 1. prompt design, 2. LLM conditioning, and 3. evaluation metrics. Together, these components guarantee the efficiency and reproducibility of our method.

\subsection{Prompt Design}
\label{sec:method:prompt}

% \YY{Introduce how we design prompt for this task:
%     \begin{enumerate}
%         \item The overview of the prompt design
%         \item How role-play and questionnaire are used in the prompt design, echo to exp
%         \item show the importance and significance of this design
%     \end{enumerate}
% }

% Prompt design is a crucial aspect of our framework, as it determines the prediction objective as well as information provided to the LLMs for predicting personality traits. In general, our prompt includes following information: 1. Background information: introduction to the task and the role settings; 2. Counseling dialogues: the dialogues between the counselor and the client are provided as part of the prompt; 3. Prediction objective: following the counseling dialogues, the LLMs are prompted to predict the BFI traits of the client based on the dialogues.
% Prompt design is a crucial aspect of our framework, as it determines both the prediction objective and the information provided to the LLMs for predicting personality traits. Our prompt design includes the following components:
The construction of prompts is essential, as it sets the objective of tasks and organizes the information for LLM to predict personality traits. Here, we outline our systematic method for prompt design:

% \indent \textbf{1. Background Information:} An overview of the task and role settings in the 'system prompt'.
\noindent \textbf{1. Background Information:} We commence with a 'system prompt' that delineates the contextual framework and defines the role of LLM, thereby ensuring a consistent initiation of the interaction. \\
% \indent \textbf{2. Counseling Dialogues:} The conversations between the counselor and the client.,
\noindent \textbf{2. Counseling Dialogues:} The dialogues between counselor and client furnish LLM with essential contextual information for conditioning. \\
% \indent \textbf{3. Prediction Objective:} After the dialogues, the LLMs are asked to predict the BFI traits of the client based on the interactions.
\noindent \textbf{3. Prediction Objective:} Items from BFI questionnaires is integrated into prompt to guide LLM to predict the BFI traits with Psychology prior.


% Inspired by previous works~\cite{wang2024incharacter,jiang2024personallm}, we adopt a role-play strategy to let LLM simulate the client in counseling dialogues. With the prior that LLM can simulate the client's activity in counseling, it can better understand the client's personality traits and fill the questionnaire as the client.
% Inspired by previous works~\cite{wang2024incharacter,jiang2024personallm}, we adopt a role-play strategy allowing the LLM to simulate the client in counseling dialogues. By simulating the client's activities during counseling, the LLM can better understand the client's personality traits and complete the questionnaire as if it were the client.
Building on the foundation of previous studies~\cite{wang2024incharacter,jiang2024personallm}, our study pioneers the use of a role-play strategy in counseling sessions, allowing the LLM to better understand the client and then accurately complete the questionnaire on behalf of the client.

% With this in mind, we involve questionnaire item within the prompt. No like previous works~\cite{pan2023llms,huang2023chatgpt,rao2023can} who use MBTI tests, we use the Big Five Inventory (BFI) questionnaire~\cite{john1991big} instead, which has a greater scientific validity and reliability as well as fine-graind traits. The questionnaire items are provided to the LLMs at the end of the counseling dialogues, and the LLMs are asked to fill in the questionnaire based on the dialogues.
% Additionally, we integrate questionnaire items within the prompt. Unlike prior works~\cite{pan2023llms,huang2023chatgpt,rao2023can} that utilize MBTI tests~\cite{myers1962myers}, we employ the BFI questionnaire~\cite{john1991big} due to its greater scientific validity, reliability, and fine-grained trait measurement. The questionnaire items are provided to the LLMs at the end of the prompt, and the LLMs are asked to complete the questionnaire based on the dialogues as task objective. A prompt template for client is presented as follows:

Furthermore, we integrate the BFI questionnaire~\cite{john1991big} as an objective. In contrast to MBTI utilized in previous studies~\cite{pan2023llms,huang2023chatgpt,rao2023can}, the BFI is chosen for its superior scientific reliability and validation to assess detailed personality traits, with an in-depth discussion provided in Sec.~\ref{sec:appendix:questionnaire}. This inclusion is essential for aligning the LLM's outputs with validated psychological evaluations, thereby improving the accuracy and relevance of the predictions.

A client prompt is presented as follows:

% system_prompt = """Act like a real human and do not mention anything with AI. 表现得像个真正的人类，不要提及任何与人工智能有关的事情。作为这次心理咨询的来访者，你将与你的咨询师进行对话。"""
% """在本次心理咨询结束之前，请根据聊天内容与你自身的情况完成下面这道选择题：
% ---
% 题目：{}
% 选项：
% 1. 非常不同意
% 2. 不太同意
% 3. 中立
% 4. 比较同意
% 5. 非常同意
% ---
% 请告诉我你的选项并说明理由："""

\noindent \fbox{%
    \begin{minipage}{\dimexpr\linewidth-2\fboxsep-2\fboxrule\relax}
        \small
        \textbf{System Prompt:} Act like a real human and do not mention anything with AI. Act as the client in this counseling session, you will have a conversation with your counselor. \\
        --- \\
        \textbf{User:} \{utterance 1 from counselor\} \\
        \textbf{Assistant:} \{utterance 1 from client\} \\
        \textbf{User:} \{utterance 2 from counselor\} \\
        \textbf{Assistant:} \{utterance 2 from client\} \\
        ... \\
        \textbf{User:} Before we end today's counseling session, please complete the following questionnaire based on the conversation and your own situation: \\
        --- \\
        \textbf{Question:} \{item from BFI questionnaire\} \\
        \textbf{Options:} \\
        \textit{1. Disagree (strongly)} \\
        \textit{2. Disagree (a little)} \\
        \textit{3. Neutral (no opinion)} \\
        \textit{4. Agree (a little)} \\
        \textit{5. Agree (strongly)} \\
        --- \\
        Please tell me your choice and explain the reason:
    \end{minipage}%
    %   \captionof{InfoBox}{Here is my caption\label{fg:A}}
}

This combined method increases the model's ability to produce contextually fitting responses, thus enhancing the effectiveness of predictions. The complete prompt and BFI questionnaire items can be found in Sec.~\ref{sec:appendix:prompt_lists} and Sec.~\ref{sec:appendix:questionnaire}, respectively.

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=\linewidth]{example-image-golden}
%     \caption{Promtpt Example}
%     \label{fig:prompt_example}
% \end{figure}




\subsection{LLM Conditioning for BFI Trait Prediction}
\label{sec:method:llm}

% \input{tables/model_ablation.tex}
\begin{table*}[t]
    \centering
    \resizebox{\linewidth}{!}{
        \begin{tabular}{llllllr}
            \toprule
                                                                & Open Mindedness   & Conscientiousness & Extraversion      & Agreeableness     & Negative Emotionality & Avg.           \\
            Model                                               &                   &                   &                   &                   &                       &                \\
            \midrule
            GPT-4-turbo~\cite{openai2023gpt4}                   & 0.407***          & 0.360**           & 0.507***          & 0.303*            & 0.337**               & 0.383          \\
            gemini-1.5-pro-latest~\cite{geminiteam2024gemini}   & 0.521***          & 0.438***          & 0.494***          & 0.356**           & 0.314**               & 0.425          \\
            gemini-1.5-flash-latest~\cite{geminiteam2024gemini} & 0.304*            & 0.357**           & 0.248*            & 0.358**           & 0.320**               & 0.317          \\
            gemini-1.0-ultra-latest~\cite{geminiteam2024gemini} & 0.412***          & 0.316**           & 0.372**           & 0.057             & 0.309*                & 0.293          \\
            gemini-1.0-pro-001~\cite{geminiteam2024gemini}      & 0.366**           & 0.309*            & 0.320**           & 0.117             & 0.294*                & 0.281          \\
            DeepSeek-Chat~\cite{deepseekai2024deepseek}         & 0.443***          & 0.385**           & 0.434***          & 0.337**           & 0.379**               & 0.396          \\
            qwen-long~\cite{bai2023qwen}                        & 0.346**           & 0.376**           & 0.451***          & 0.265*            & 0.405***              & 0.369          \\
            qwen-turbo~\cite{bai2023qwen}                       & 0.363**           & 0.314**           & 0.418***          & 0.279*            & 0.321**               & 0.339          \\
            ERNIE-Speed-128K~\cite{ernie}                       & 0.138             & 0.167             & 0.241*            & -0.203            & 0.239*                & 0.116          \\
            ERNIE-Lite-8K-0308~\cite{ernie}                     & -0.118            & -0.030            & 0.148             & -0.237            & 0.285*                & 0.010          \\
            \midrule
            Qwen1.5-110B-Chat~\cite{bai2023qwen}                & 0.457***          & 0.480***          & 0.562***          & 0.412***          & 0.561***              & 0.494          \\
            % Qwen2-72B-Instruct                                  & 0.480***          & 0.346**           & 0.471***          & 0.326**           & 0.373**               & 0.399          \\
            Qwen-72B-Chat~\cite{bai2023qwen}                    & 0.480***          & 0.470***          & 0.510***          & 0.400***          & 0.516***              & 0.475          \\
            Meta-Llama-3-70B-Instruct~\cite{llama3}             & 0.368***          & 0.497***          & 0.492***          & 0.375***          & 0.369***              & 0.420          \\
            deepseek-llm-67b-chat~\cite{deepseekai2024deepseek} & 0.312**           & 0.412***          & 0.476***          & 0.301**           & 0.444***              & 0.389          \\
            % Yi-1.5-34B-Chat~\cite{ai2024yi}                     & 0.350**           & 0.369***          & 0.451***          & 0.242*            & 0.328**               & 0.348          \\
            Yi-34B-Chat~\cite{ai2024yi}                         & 0.456***          & 0.440***          & 0.544***          & 0.324**           & 0.350**               & 0.423          \\
            AquilaChat2-34B        \cite{Aquila2}               & 0.110             & 0.119             & 0.188             & 0.022             & 0.206                 & 0.129          \\
            internlm2-chat-20b     \cite{cai2024internlm2}      & 0.240*            & 0.345**           & 0.434***          & 0.221             & 0.206                 & 0.289          \\
            Baichuan2-13B-Chat~\cite{yang2023baichuan}          & 0.059             & -0.044            & 0.029             & 0.070             & 0.237*                & 0.070          \\
            glm-4-9b-chat~\cite{zeng2023glmb}                   & 0.293*            & 0.312**           & 0.240*            & 0.036             & 0.305*                & 0.237          \\
            gemma-1.1-7b-it~\cite{gemmateam2024gemma}           & 0.125             & 0.169             & 0.329**           & 0.037             & 0.070                 & 0.146          \\
            \midrule
            Meta-Llama-3-8B-Instruct~\cite{llama3}              & 0.177             & 0.434***          & 0.233             & 0.111             & 0.303*                & 0.252          \\
            Meta-Llama-3-8B-Instruct-BFI (Ours)                 & \textbf{0.692***} & \textbf{0.554***} & \textbf{0.569***} & \textbf{0.448***} & \textbf{0.648***}     & \textbf{0.582} \\
            % Qwen1.5-7B-Chat~\cite{bai2023qwen} & 0.011 & 0.129 & 0.127 & 0.091 & 0.216 & 0.115 \\
            % Qwen1.5-7B-Chat-anonymous-BFI-0603-2 & 0.562*** & 0.470*** & 0.537*** & 0.378*** & 0.558*** & 0.501 \\
            % Qwen2-7B-Instruct & 0.266* & 0.309* & 0.425*** & 0.109 & 0.261* & 0.274 \\
            % Qwen2-7B-Instruct-anonymous-BFI & 0.502*** & 0.389*** & 0.502*** & 0.460*** & 0.557*** & 0.482 \\
            \bottomrule
        \end{tabular}
    }
    \caption{Correlation of Predicted and Actual BFI Traits across Various LLMs. The models include state-of-the-art proprietary models such as GPT-4, gemini, and several open-source models such as Llama3, Qwen, Yi, etc. The results highlight the variability in predictive validity across models, with certain models, particularly the fine-tuned Meta-Llama-3-8B-Instruct-BFI (ours) models, showing notably higher correlation coefficients, demonstrating the highest overall performance, underscoring the efficacy of our tailored fine-tuning approach. Significance levels are denoted by * (p-value < 0.05), ** (p-value < 0.01), and *** (p-value < 0.001), indicating robust statistical support for observed correlations.
    }
    \label{tab:model_ablation}

\end{table*}



% \YY{With generated prompts, show how we leverage LLMs to predict BFI traits}

% The cornerstone of our method is the conditioning of LLMs to predict personality traits, leveraging their advanced text generation capabilities. This process is predicated on the strategic provision of contextually relevant prompts to guide the model's output. The mathematical representation of this text generation process is encapsulated by the equation:

% \begin{equation}
%     y_{BFI} = \text{LLM}(x_{context}, \text{prompt})
% \end{equation}

% Here, $x_{context}$ represents the historical counseling dialogue, while $\text{prompt}$ is a query derived from the BFI questionnaire. To simulate a counseling scenario, the dialogue history is transformed into a multi-turn format congruent with the LLM's conversational framework. The client question is seamlessly integrated into the prompt, tasking the LLM with generating a response that not only answers the query based on the provided context but also elucidates the reasoning behind its choice. This response, denoted as $y_{BFI}$, is then analyzed to extract the BFI trait assessment, which is subsequently used to compute the client's personality profile according to the standard scoring methodology of the client.

The cornerstone of our method is conditioning LLMs to predict BFI traits by leveraging their advanced text comprehension and generation capabilities. This process involves strategically providing contextually relevant prompts to guide the model's output, encapsulated in the following equation:

\begin{equation}
    \begin{aligned}
        y_{\text{BFI}} = \text{LLM}(x_{\text{context}}, \text{questionnaire})
    \end{aligned}
    \label{eq:llm}
\end{equation}

In this equation, \( x_{\text{context}} \) signifies the historical counseling dialogue, while \( \text{questionnaire} \) refers to an item of the BFI questionnaire. To mimic a counseling scenario, the dialogue history is structured into a chat history format that aligns with the LLM's data format. The prediction objective guiding the LLM to produce a response that not only addresses the item based on the given context but also explains the rationale behind its selection. This response, labeled \( y_{\text{BFI}} \), is then examined to derive the BFI trait assessment using a regex of keywords to extract the choice, which is then utilized to calculate the client's personality profile according to standard BFI scoring methods.

% Several factors influence the prediction validity of the LLM, including the type of LLM, its scale, and the granularity of the provided context. The type of LLM affects the model's language comprehension and generation abilities. Additionally, the scale of the LLM, which refers to its size and computational power, plays a crucial role in the quality and accuracy of the predictions. Granularity pertains to the extent of context provided in the prompts, with more detailed context typically enhancing the model's predictive capabilities.
Given that various factors affect the validity of predictions, such as the type of LLM, its scale, and the granularity in the provided context,
% To determine the impact of these factors on prediction validity, 
we conduct a comparative analysis for each factor in Sec.~\ref{sec:exp:rq1}.


\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/granularity.png}
    \caption{The impact of granularity of the progress of the session on the prediction validity.}
    \label{fig:granularity}
\end{figure}

% \YY{Disscuss how different factors of LLM that will affect the prediction, such as type, scale, granularity of context/prompt}

\subsection{Evaluation Metrics}

% \YY{Show only necessary metrics for following experiments, move the others to appendix}

% % To ensure the robustness and applicability of our proposed method, we adopt a comprehensive suite of metrics aimed at evaluating both the validity and reliability of the LLMs in predicting the BFI traits. This section delineates the specific metrics employed in our study, underscoring their significance in psychological assessment.

% \subsubsection{Reliability Metrics}
% % Reliability, in the context of psychological assessments, denotes the consistency and stability of a test across multiple administrations. A reliable test consistently reflects the true psychological characteristic it aims to measure, rather than being influenced by random error or variability. This concept is paramount in our evaluation to ascertain that the LLMs are not merely "Stochastic Parrots" but are genuinely reflective of the BFI traits. We utilize two primary metrics for assessing reliability:

% \noindent 1.\textit{Internal Consistency:} This metric evaluates the degree of correlation among individual test items, ensuring that they collectively measure the same construct. We employ Cronbach's Alpha ($\alpha$) as the statistical measure for internal consistency. A higher $\alpha$ value indicates a more reliable construct measurement, with values above 0.7 generally considered acceptable in psychological research.

% % \noindent 2.\textit{Test-Retest Reliability:} To measure the stability of our method over time, we apply the Kappa statistic, which assesses the consistency of test results upon repeated administrations under similar conditions. A higher Kappa value suggests greater reliability, indicating that the LLMs' predictions of the BFI traits are stable over time.

% \YY{Test-retest is twaddle... discuss in the appendix, report standard deviation instead}

% \noindent 2.\textit{Test-retest Reliability:} To measure the stability of our method over time, we report the standard deviation of the predicted scores for each trait across multiple runs. A lower standard deviation indicates greater stability and reliability in the LLMs' predictions of the BFI traits.

% \subsubsection{Validity Metrics}
% % Following the establishment of reliability, we proceed to examine the validity of our method, which pertains to the accuracy and relevance of the test in measuring the intended construct. We focus on two types of validity:

% \YY{proof for effectiveness of the framework}

% \noindent 1.\textit{Criterion Validity:} This form of validity assesses the correlation between the test outcomes and a pre-established benchmark or 'criterion.' In our study, the ground truth data for the BFI traits serve as this criterion. To quantify criterion validity, we employ the Pearson correlation coefficient to evaluate the strength and direction of the association between predicted and actual personality traits. A higher Pearson coefficient, coupled with a statistically significant p-value, indicates a strong and meaningful correlation. Additionally, we calculate the Mean Absolute Error (MAE) between the predicted scores and the actual scores for each question of the assessment. A lower MAE signifies a closer alignment with the ground truth, thereby indicating higher predictive validity.

% \noindent 2.\textit{Content Validity:} This metric evaluates the extent to which the LLMs' predictions encompass the full range of the BFI traits dimensions. We conduct a qualitative analysis of both the most accurate and the least accurate predictions to uncover the underlying reasons for their performance. By examining the dimensions where predictions align closely with the ground truth as well as those where discrepancies occur, we gain insights into the content validity of our method.
% % This analysis includes a detailed review of the 50 least accurate predictions to identify common patterns or characteristics that may affect the LLMs' performance.

% \YY{TODO: shorten it}

% To ensure the robustness and applicability of our proposed method, we evaluate the validity and reliability of proposed framework.
To ensure the effectiveness of our framework, we further evaluated the validity and reliability.
% \paragraph{Validity} measures the accuracy and relevance of the test. \textit{1.Criterion Validity} is evaluated using the Pearson correlation coefficient and Mean Absolute Error (MAE), where higher Pearson coefficients and lower MAE signify greater accuracy. \textit{2.Content Validity} is assessed by analyzing the range of BFI trait predictions, examining both the most and least accurate predictions to gain insights into performance patterns.
% \paragraph{Validity} measures the accuracy and relevance of the test. \textit{1. Criterion Validity} is evaluated using the Pearson correlation coefficient and Mean Absolute Error (MAE), where higher Pearson coefficients and lower MAE signify greater accuracy. \textit{2. Content Validity} is assessed by analyzing the range of BFI trait predictions, examining both the most and least accurate predictions to gain insights into performance patterns.
\paragraph{Validity} Validity measures the accuracy and relevance of the test. We consider two aspects:

\textit{1. Criterion Validity} is evaluated using the Pearson correlation coefficient and Mean Absolute Error (MAE). Higher Pearson coefficients and lower MAE values indicate greater accuracy.

\textit{2. Content Validity} is assessed by analyzing the range of BFI trait predictions. We examine both the most and least accurate predictions to gain insights into performance patterns.

% \paragraph{Reliability} ensures consistency in psychological assessments. We use two primary metrics: \textit{1.Internal Consistency}, assessed with Cronbach's Alpha ($\alpha$), where values above 0.7 indicate reliability, and \textit{2.Test-Retest Reliability}, measured by the standard deviation of predicted scores across multiple runs, with lower values indicating higher stability.

% We further investigate the reliability with the internal consistency and test-retest reliability metrics, which are detailed in Sec.~\ref{sec:appendix:reliability}.
\paragraph{Reliability} We investigate reliability through internal consistency and test-retest reliability, which are elaborated in Sec.~\ref{sec:appendix:reliability} for space constrains.

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/correlation_model_size_plot.png}
    \caption{Correlation varies by model size.}
    \label{fig:correlation_model_size}
\end{figure}

% \YY{Add perplexity for LLM's performance?}

% By leveraging these meticulously chosen metrics, our study aims to rigorously evaluate and validate the capability of LLMs in accurately predicting the BFI traits based on counseling dialogues. The subsequent sections will elaborate on our innovative approach to simulating counseling interactions and detail the methodology employed to ensure the accuracy and reliability of our predictions.

% \begin{figure*}[ht]
%     \centering
%     \includegraphics[width=\textwidth]{figures/correlation_roles.png}
%     \caption{The relationship between the predicted and actual BFI traits varies by role using Qwen1.5-72b-Chat~\cite{bai2023qwen}. The accuracy of predictions is notably enhanced by role-play. The client role shows the strongest correlation. * indicates p-value < 0.05, ** indicates p-value < 0.01, *** indicates p-value < 0.001.}
%     \label{fig:correlation_roles}
% \end{figure*}

% \begin{table}
%     \centering
%     \resizebox{\linewidth}{!}{
%         \begin{tabular}{llllll}
%             \toprule
%             %    & Open Mindedness & Conscientiousness & Extraversion & Agreeableness & Negative Emotionality \\
%                        & O        & C        & E        & A       & N        \\
%             Model Size &          &          &          &         &          \\
%             \midrule
%             0.5B       & -0.165   & 0.174    & -0.097   & -0.083  & -0.016   \\
%             1.8B       & 0.154    & 0.067    & 0.197    & 0.089   & 0.101    \\
%             4B         & 0.189    & 0.107    & 0.313**  & 0.052   & 0.075    \\
%             7B         & 0.309**  & 0.336**  & 0.304**  & 0.158   & 0.390*** \\
%             14B        & 0.356**  & 0.468*** & 0.475*** & 0.334** & 0.495*** \\
%             32B        & 0.402*** & 0.334**  & 0.439*** & 0.293*  & 0.315**  \\
%             72B        & 0.491*** & 0.449*** & 0.542*** & 0.350** & 0.531*** \\
%             \bottomrule
%         \end{tabular}
%     }
% \end{table}



==> sec/4.experiments.tex <==
\section{Experiments}

% To assess the effectiveness of our proposed framework, we conduct a series of experiments designed to evaluate the validity and reliability of LLMs in predicting BFI traits from counseling dialogues. As we are the first to explore this research direction, setting different baselines for answering our research questions is essential. We structure our experiments around three primary research questions (RQs), each designed to systematically evaluate the performance of our proposed framework.
To assess the effectiveness of our proposed framework, we conducted a series of experiments designed to evaluate the validity. Our experiments are structured around three primary research questions (RQs), each formulated to systematically evaluate the performance of our framework.

\subsection{Research Questions}
% Echo to our pivotal question in the section\ref{sec:intro}, we structure our investigation around three research questions (RQs), each designed to explore the capabilities of LLMs in predicting BFI traits from psycho-counseling dialogues:
Building on the pivotal question outlined in Sec.~\ref{sec:intro}, we structure our investigation around the following research questions:

\vspace{0.2cm}

% \YY{RQ1: proof for effectiveness\\
%     RQ2: error analysis\\
%     RQ3: fine-tuning a new model}

% \noindent \textbf{RQ1:} \textit{Can LLMs predict BFI traits in psycho-counseling dialogues?}\\
% % \noindent \textbf{RQ2:} \textit{What is the impact of dialogue session characteristics on the validity?}\\
% % \noindent \textbf{RQ3:} \textit{How do individual differences among clients influence the validity?}
% \noindent \textbf{RQ2:} \textit{How do different characteristics impact the validity of BFI trait prediction?}\\
% \noindent \textbf{RQ3:} \textit{Will fine-tuning a new model benefit the prediction validity?}

% \noindent \fbox{
%     \begin{minipage}{\dimexpr\linewidth-2\fboxsep-2\fboxrule\relax}
%         \noindent \textbf{RQ1:} \textit{Can LLM predict BFI traits from dialogues?} \\
%         \indent \indent  -- \textbf{Validity of proposed framework} \\
%         \noindent \textbf{RQ2:} \textit{What influences the validity of predictions?} \\
%         \indent \indent  -- \textbf{Error Analysis} \\
%         \noindent \textbf{RQ3:} \textit{How to align a LLM in predicting BFI traits?} \\
%         \indent \indent  -- \textbf{Fine-tune LLM for BFI Prediction} 
%     \end{minipage}
% }

\noindent \textbf{RQ1:} \textit{Can LLM predict BFI traits from dialogues?} \\
\indent \indent  -- \textbf{Validity of proposed framework}

\noindent \textbf{RQ2:} \textit{What influences the validity of predictions?} \\
\indent \indent  -- \textbf{Error Analysis}

\noindent \textbf{RQ3:} \textit{How to align a LLM in predicting BFI traits?} \\
\indent \indent  -- \textbf{Fine-tune LLM for BFI Prediction}

The questions we pose shape our experimental design, allowing for a structured assessment of how well our proposed framework performs.

% \subsection{Experimental Setup}

% Our experimental design is tailored to systematically address each research question through a sequence of carefully planned studies.

% \YY{Echo to each RQ, show how we design the experiments}

% \YY{RQ1: validate the effectiveness of the framework, including:
%     \begin{enumerate}
%         \item (Prompt Engineering) why use role-play and questionnaire?
%         \item (Prompt Engineering) how does different role affect the prediction (client, counselor, observer)? will assigning specific roles to the model help? (Compute reliability for recheck)
%         \item (Prompt Engineering) how does the granularity of context/prompt affect the prediction?
%         \item (Ablation) how does different type, scale affect the prediction? full vs anonymous?
%     \end{enumerate}
% }

% % \paragraph{For RQ1,} we want to assess the validity of LLM predictions in predicting BFI traits in psycho-counseling dialogues. To this end, we first establish a baseline predicting BFI traits directly from the dialogues. Then we extend our simulations to 1. include the roles of client, counselor, and observer. 2. leverage the questionnaire of client to guide the LLMs in predicting the BFI traits. 3. employ different state-of-the-art LLMs, to evaluate the performance of different models in predicting the BFI traits. The results of these experiments will secure a comprehensive understanding of the LLMs' predictive capabilities.

% \YY{RQ2: Error analysis, including:
%     \begin{enumerate}
%         \item general analysis of the error with MAE, indentify outliers in session-level and client-level for further error analysis
%         \item (session-level) error analysis insights: limited context, lack of information, etc.
%         \item (user-level) error analysis insights: individual differences, social/self-presentation bias, etc.
%     \end{enumerate}
%     show strengths and boarders of our framework
% }

% % \paragraph{For RQ2,} we want to delve into the impact of different dialogue session on the performance of predicting. We first analysis the granularity of the progress of the session, from 20\% to 100\% of the session, to see how the prediction validity changes. Then we analysis the error between the predicted and actual BFI traits for each dimension with different session to see the impact of the session on the prediction validity and identify the potential factors contributing to inaccuracies.

% \YY{RQ3: Fine-tuning a new model, including:
%     \begin{enumerate}
%         \item limitations of the current model: effectiveness, efficiency, etc.
%         \item how to fine-tune a new model?
%         \item evaluate the performance of the fine-tuned model
%         \item ablation on different fine-tuning settings (w/, w/o questionnaire, resoning, DPO, SFT)
%     \end{enumerate}
% }

% % \paragraph{For RQ3,} we aim to investigate the influence of individual differences on the prediction validity of BFI traits. We conduct an error analysis to identify the clients with the highest and lowest prediction validity, examining the characteristics of these clients to determine the factors that may influence the LLMs' performance. This analysis will provide valuable insights into the individualized performance of LLMs in predicting personality traits.

\subsection{Data Collection and Preprocessing}

% We collect 853 counseling dialogues from 82 adults clients (55 females, 19- to 54-year-olds, M=27.62 years, SD=5.94) and 9 counselorss (7 females, Mean age=34.67 years old, SD=7.45), the statistics of the counseling dialogues are shown in Table\ref{tab:statistics_dialogues}. 
We gathered 853 counseling dialogues from 82 adult clients (55 females, age range 19-54 years old, M=27.62 years old, SD=5.94) and 9 counselors (7 females, age range 25-45, M=34.67 years old, SD=7.45), summarized in Tab.~\ref{tab:statistics_dialogues}.
% Before their first session, clients completed the BFI questionnaire with the Chinese version of the BFI-2 questionnaire~\cite{soto2017next}. This allowed us to correlate the subsequent dialogue analysis with established personality profiles.
Before their initial sessions, clients completed the Chinese version for BFI-2 questionnaire~\cite{soto2017next}, linking dialogue analyses with established personality profiles.

% We split about 30\%(242) of the dialogues into validation sets, and the remaining 70\%(611) into training sets. To ensure privacy when using proprietary LLMs, we manually anonymized validation split (46 females, M=27.84 years, SD=6.34), by replacing personally identifiable information with placeholders. This step was crucial to maintain ethical standards and compliance with data protection regulations.
Approximately 30\% (242) of the dialogues were allocated to the validation set, with the remaining 70\% (611) used for training. We anonymized the validation set manually to ensure privacy, replacing all personally identifiable information with placeholders. This step underscores our commitment to ethical standards and data protection compliance.

% \YY{Collecting human observer rating results (true\_observer), for what?\\
%     1. Criterion validity for observer (pred\_observer vs true\_observer), also compare (pred\_client vs true\_observer) and (pred\_counselor vs true\_observer) for observer rating settings?\\
%     2. Proof for social desirability bias, compare (true\_client vs true\_observer) and (true\_counselor vs true\_observer) for observer rating settings?\\
%     How to validate the reasoning results of LLM, also human rating?
% }

% % Prior to their initial counseling session, clients were administered the BFI questionnaire with the Chinese verion of BFI-2 questionnaire~\cite{soto2017next}, ensuring subsequent dialogue analysis could be correlated with established personality profiles. To facilitate the use of proprietary LLMs while safeguarding privacy, we manually anonymized 242 (46 female, mean age=27.84 years, SD=6.34) of these sessions, meticulously excising any personally identifiable information. The dialogues were reformatted into an interleaved structure, alternating between client and counselor contributions, to mimic the natural flow of conversation. This processed dataset served as the foundation for conditioning the LLMs, providing them with a rich historical context for simulation and analysis.

% The processed dataset was formatted into an interleaved structure, alternating between client and counselor contributions. This structure reflects the natural flow of conversation, allowing LLMs to simulate and analyze counseling scenarios effectively.

% \subsection{RQ1: Can LLMs effectively predict BFI traits from counseling dialogues?}
\subsection{RQ1: Validity of Proposed Framework}
\label{sec:exp:rq1}
% \YY{RQ1: validate the effectiveness of the framework, including:
%     \begin{enumerate}
%         \item (Prompt Engineering) why use role-play and questionnaire?
%         \item (Prompt Engineering) how does different role affect the prediction (client, counselor, observer)? will assigning specific roles to the model help? (Compute reliability for recheck)
%         \item (Prompt Engineering) how does the granularity of context/prompt affect the prediction?
%         \item (Ablation) how does different type, scale affect the prediction? full vs anonymous?
%     \end{enumerate}
% }

% To validate the effectiveness of our framework, we conducted a series of experiments, including employing different methods for prompt engineering, role-play, and questionnaire integration. We also evaluated the impact of different LLM types and scales on prediction validity echo to equation \ref{eq:llm}.

% To validate the effectiveness of our proposed framework, we designed a comprehensive experimental setup. This included varied approaches to prompt engineering, role-playing, and the integration of questionnaires, assessing the impact of these methods on the accuracy of predicting the BFI traits using different types and scales of LLMs as detailed in Equation~\ref{eq:llm}.
To evaluate effectiveness, we conducted a series of experiments incorporating various methods such as prompt engineering, role-play, and questionnaire integration. Furthermore, we evaluated the impact of different LLM types and scales on prediction validity, as described in Eq.~\ref{eq:llm}.

% \YY{Answer ``Why use role-play and questionnaire?''}
\paragraph{Methods for prediction}
% We first establish a baseline of directly predicting BFI traits from dialogues and without using any tricks. Then, we extend our settings to include the role-play strategy and questionnaire integration. The results are shown in Table\ref{tab:method_ablation}. 
Initially, we established a baseline for predicting BFI traits directly from dialogues without additional strategies.
Subsequently, we extended our approach to include role-play strategies and questionnaire integration to validate the effectiveness of our framework.
% Introduce the results, and interpret the results.
% We first established a baseline for predicting BFI traits directly from dialogues without any additional strategies. Subsequently, we extended our settings to include role-play strategies and questionnaire integration. The results are shown in Tab.~\ref{tab:method_ablation}.
% The baseline performance was poor, but the role-play strategy with questionnaire integration significantly enhanced prediction validity. Consistenting with the principles of Item Response Theory~\cite{baker2001basics,reise2009item,embretson2013item}, it's hard to measure personality directly, so tools like questionnaire are needed and involving Role-Play strategy can help LLMs to better understand the context and answer the BFI questionnaire.
The results, presented in Tab.~\ref{tab:method_ablation}, indicate that the baseline performance was suboptimal.
However, the incorporation of role-play strategies with questionnaire integration significantly enhanced prediction validity.
Consistent with the principles of Item Response Theory~\cite{baker2001basics,reise2009item,embretson2013item}, it is challenging to measure personality directly; therefore, tools such as questionnaires are necessary, and incorporating role-play strategies helps LLMs better understand the context and respond accurately to the BFI questionnaire.

% \YY{Answer ``How does different role affect the prediction?''}
% Ablation of roels in role-play strategy, including client, counselor, and observer. Reuslts are shown in Tab.\ref{tab:role_ablation}. Extend ablation of assigning specific roles to the model, including famous Psychologists, shown in Tab.\ref{tab:role_ablation_extend} in appendix.
\paragraph{Role Impact}
% While the baseline performance is poor, the role-play strategy with questionnaire integration significantly enhances prediction validity. We further explore the impact of different roles, including client, counselor, and observer, on prediction validity. 
% Role-Play strategy with questionnaire integration significantly enhances prediction validity, and it comes a nature question that ``\textit{Does every role have the same impact?}'' we conducted ablation studies involving different roles, including client and counselor, the native participants in counseling, and observer, an external rater.
The role-play strategy, when combined with questionnaire integration, notably improves prediction validity. This raises the question, “\textit{Do all roles have the same effect?}” To investigate, we performed ablation studies on various roles, including client, counselor (the primary participants in counseling), and observer (an external evaluator).
% The results are shown in Tab.~\ref{tab:role_ablation}.
% All three roles significantly enhance prediction validity compared to the no-role baseline.
The results, shown in Tab.~\ref{tab:role_ablation}, indicate that the three roles significantly enhance the validity of the prediction compared to the baseline without role.
% The client role exhibits the strongest correlation.
% This result prompts us that in role-play tasks, the closer the role is to the task itself, the higher the task performance.
The client role exhibits the strongest correlation, suggesting that roles closer to the task itself yield higher performance.
% We further extended the ablation study to include 10 famous psychologists, 4 common name and 1 random name as roles, the results are shown in Tab.~\ref{tab:role_ablation_extend} in the appendix.
We further extended the ablation study to include ten famous psychologists, four common names, and one random name as roles. The results, shown in Tab.~\ref{tab:role_ablation_extend} in the Appendix, indicate that assigning specific roles does not provide any additional benefit.
% \YY{Answer ``How does the granularity of context/prompt affect the prediction?''}
% Ablation of granularity of context/prompt, including 10\% to 100\% of the session. Results are shown in Fig.\ref{fig:granularity}.
% \paragraph{Granularity} Granularity means the progress of a counseling session, it is a key factor to determin how much context information is needed for the LLM to predict the BFI traits.
\paragraph{Granularity of Context}
Granularity refers to the progression of a counseling session and determines the extent of contextual information required for the LLM to accurately predict BFI traits.
% We conducted ablation studies involving different granularity of context/prompt, from 10\% to 100\% of the session.
% The results are shown in Fig.\ref{fig:granularity}.
% The prediction validity increases as the session progresses, with the highest validity achieved at 100\% of the session.
We conducted ablation studies involving different granularities of context/prompt, ranging from 10\% to 100\% of the session.
% The results, presented in Fig.\ref{fig:granularity}, indicate that prediction validity increases as the session progresses, with the highest validity achieved at 100\% of the session.
As illustrated in Fig.~\ref{fig:granularity}, 40\% of the session marks a critical threshold.
Before this point, prediction validity is unstable; beyond it, validity and significance stabilize.
These results suggest that in our framework, the LLM can effectively predict BFI traits with just 40\% of the session context.

% \YY{Answer ``How does different type, scale of LLM affect the prediction?''}
% Ablation of different type, scale of LLMs, results are shown in Tab.\ref{tab:model_ablation}.
% \paragraph{Models} Echo to equation \ref{eq:llm}, the performance of LLM is another key factor to determine the validity.
\paragraph{Models}
% As per equation~\ref{eq:llm}, the performance of LLMs is a key factor in determining validity.
As referenced in Eq.~\ref{eq:llm}, the effectiveness of LLMs is pivotal in validating the predictions of the BFI traits.
% We conducted ablation invloding 20 proprietary and open-sourced cutting-edge LLMs as well as a fine-tuned LLama3 by us to evaluate the performance of different models in predicting the BFI traits.
Our study evaluates a diverse set of 20 state-of-the-art proprietary and open-source LLMs, including a custom fine-tuned version of LLama3, to ascertain their predictive accuracy regarding the BFI traits.
% The results are shown in Table\ref{tab:model_ablation}.
Tab.~\ref{tab:model_ablation} summarizes the findings.
% Gemini-1.5-pro~\cite{geminiteam2024gemini} exhibits the highest validity in proprietary LLMs with a average Person correlation of 0.425 on all traits and Qwen1.5-110B-Chat~\cite{bai2023qwen} shows the highest validity in open-sourced LLMs with a average Person correlation of 0.494 on all traits.
Among the proprietary models, Gemini-1.5-pro~\cite{geminiteam2024gemini} demonstrated the most robust performance, achieving an average Pearson correlation of 0.425 for all traits.
In contrast, Qwen1.5-110B-Chat~\cite{bai2023qwen} led among open-source models with an average Pearson correlation of 0.494.
In particular, our analysis reveals that models with capacities exceeding 34 billion parameters exhibit statistically significant correlations.
% With observation that only models over 34B could show statistically significant correlation, we further investigate the correlation between model size and prediction validity by employing Qwen1.5 family of 4B to 110B models. The results are shown in Fig.~\ref{fig:correlation_model_size}. The validity of predictions increases with model size, consistent with the Scaling Laws~\cite{kaplan2020scaling} in LLMs. We present the full per-dimension Preason correlation results in Sec.~\ref{sec:appendix:full_correlation_results} in the appendix.
This observation led to a further examination of the relationship between model size and predictive validity, detailed in Figure \ref{fig:correlation_model_size} using the Qwen1.5 model series ranging from 4B to 110B.
The results confirm that the predictive validity improves with increasing model size, aligning with the Scaling Laws for LLMs~\cite{kaplan2020scaling}.
Detailed per-dimension results of Pearson correlation are presented in Section~\ref{sec:appendix:full_correlation_results} in the appendix.

% \subsection{RQ2: What influences the validity of predictions?}
\subsection{RQ2: Error Analysis}
\label{sec:exp:rq2}
% \YY{RQ2: Error analysis, including:
%     \begin{enumerate}
%         \item general analysis of the error with MAE, indentify outliers in session-level and client-level for further error analysis
%         \item (session-level) error analysis insights: limited context, lack of information, etc.
%         \item (user-level) error analysis insights: individual differences, social/self-presentation bias, etc.
%     \end{enumerate}
%     show strengths and boarders of our framework
% }

% To investigate the factors influencing the validity of predictions, we conducted a comprehensive error analysis from both model and client perspectives.
To thoroughly examine the factors influencing the validity of our predictions, we conducted an extensive error analysis from both the model and client perspectives.
This analysis aimed to delineate the boundaries of our framework and provide practical insights for future research.

% explain the results of MAE, and if MAE is <1, then the model is valid because if the choice is wrong, the error is >=1.
\paragraph{Outliers}
% we first conducted a general analysis of the error with MAE and identified outliers.
% % The results are shown in Fig.\ref{fig:mae_analysis}.
Our initial step involved a general assessment of model errors using Mean Absolute Error (MAE), with results depicted in Fig.\ref{fig:mae_analysis}.
% The mean MAE of all traits is $0.474_{\pm0.191}$ within 1, further indicating the validity of the model.
The mean MAE across all traits was $0.474_{\pm0.191}$, demonstrating the overall validity of the model.
% Next, we identify outliers by Interquartile Range (IQR), outliers are identified as values that fall below $Q1 - 1.5 * \text{IQR}$ or above $Q3 + 1.5 * \text{IQR}$, where Q1 and Q3 are the first and third quartiles, respectively.
Outliers were identified using the Interquartile Range (IQR) method, where values falling below $Q1 - 1.5 *\text{IQR}$ or above $Q3 + 1.5 *\text{IQR}$ were considered outliers.
% We further conducted error analysis insights at both LLM- and client-levels to identify potential factors contributing to inaccuracies.
We then delved into error analysis at both the LLM and client levels to uncover potential factors contributing to these inaccuracies.

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=\linewidth]{figures/error_analysis_per_dimension.png}
%     \caption{Boxplot of error between predicted and actual BFI traits for each dimension and averaged over all dimensions. Red line indicates the $error=1$, which is the threshold of significant error.}
%     \label{fig:mae_analysis}
% \end{figure}

\begin{figure}[t]
    \centering
    \begin{subfigure}{.5\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/mae_analysis_qwen.png}
        \caption{Qwen1.5-110B-Chat}
        \label{fig:sub1}
    \end{subfigure}%
    \begin{subfigure}{.5\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/mae_analysis_ours.png}
        \caption{Llama3-8B-BFI(Ours)}
        \label{fig:sub2}
    \end{subfigure}
    \caption{Boxplot of MAE between predicted and actual BFI traits for each dimension and averaged over all dimensions. Red line indicates the $error=1$, which is the threshold of significant error. ``O'' indicates ``Open Mindeness'', ``C'' indicates ``Conscientiousness'', ``E'' indicates ``Extraversion'', ``A'' indicates ``Agreeableness'', ``N'' indicates ``Negative Emotionality''.}
    \label{fig:mae_analysis}
\end{figure}

\paragraph{Errors from LLMs}
% The error analysis insights at the LLM-level revealed several factors contributing to inaccuracies, including limited context, lack of information, and safety rejection of the LLM.
At the LLM level, several factors contributing to inaccuracies were identified, including limited context, insufficient information, and the safety rejections by the LLM.
% The first two factors related to the capability of the LLMs to comprehend and generate contextually appropriate responses.
The first two factors are linked to the LLM's ability to understand and generate contextually appropriate responses.
% As shown in Fig.~\ref{tab:model_ablation} and Fig.~\ref{fig:correlation_model_size}, greater model type and scale enhance prediction validity generally.
For instance, as evidenced in Fig.~\ref{tab:model_ablation} and Fig.~\ref{fig:correlation_model_size}, enhancements in model type and size generally improve prediction accuracy.
% However, some exception exists, such as the Yi-1.5 is weak than the previous version of Yi.
% However, exceptions exist, such as the Yi-1.5 and Qwen2 model performing worse than its predecessor.
% We reviewed the generated responses and found that the Yi-1.5 model tends to reject the task as saying "As a AI model, I have no personality."
% Upon reviewing the generated responses, we discovered that the Yi-1.5 and Qwen2 model often refused the task by stating, "As an AI model, I have no personality." We further investigated this safety rejection phenomenon and found that simply assigning roles might not suffice to bypass these limitations.

% We further investigated this safety rejectiong phenomenon in our task.
% We found that with only assigning the role may not be enough for the LLM to ignore the safety limitation.
% As reported in Tab.~\ref{tab:method_ablation}, only role-play and without questionnaire to directly predict BFI trails will emphasis this phenomenon, which leads to a great drop in prediction validity against the baseline.
% This motivates us to further align the LLMs with the BFI prediction task to ease the safety rejection and enhance prediction validity, we report the detailed process and result in Sec.~\ref{sec:exp:rq3}.

For safety rejections, LLM may refuse to answer the task with statements such as "As an AI model, I have no personality," which can significantly impact prediction validity. For example, ``Qwen1.5-110B-Chat'' on Tab.~\ref{tab:method_ablation} suffers 0.2\% safety rejections in direct prediction baseline, while suffers 28.09\% with only adding role-play and 0.31\% with both role-play and questionnaire. This motivates us to further align LLMs with the BFI prediction task to mitigate safety rejections and enhance prediction validity, as detailed in Sec.~\ref{sec:exp:rq3}.

\paragraph{Errors from Clients}
% ``Is our framework equally effective to every client?'' To answer this question, we conducted error analysis insights at the client-level uncovered individual differences, social/self-presentation bias, and social desirability bias as potential factors influencing prediction validity.
Addressing the question, "Is our framework universally effective across all clients?" led to an exploration of error sources at the client level.
We identified outliers using the IQR in Fig.~\ref{fig:mae_analysis} and compared the dialogues of these outliers with those of clients who have the lowest MAE to uncover potential factors affecting prediction validity. Among all the sessions predicted by Qwen1.5-110B-Chat, 15 are identified as outliers, with 2 clients having more than 75\% of their sessions indentified as outliers. Upon reviewing the dialogues, we observe that although these clients self-report high levels of open-mindedness, they consistently reject others' opinions in conversations. In addition, they struggle to articulate their own opinions clearly, often resorting to metaphors and similes to express their feelings. This discrepancy between self-reported BFI traits and actual behavior in dialogues could be attributed to social desirability bias or self-presentation bias, potentially affecting the validity of the prediction.
% Our analysis revealed that individual differences, along with social and self-presentation biases, significantly affect prediction accuracy.
% These variables introduce complexities that any robust predictive framework must account for, suggesting avenues for enhancing both the adaptability and accuracy of our system.
% \YY{Update the latest error analysis with outliers from Qwen1.5-110B and Llama3-8B-BFI(Ours) in Fig.~\ref{fig:mae_analysis}.}



% \subsection{RQ3: How to align a LLM in predicting BFI traits?}
\subsection{RQ3: Fine-tune LLM for BFI Prediction}
\label{sec:exp:rq3}
% \YY{RQ3: Fine-tuning a new model, including:
%     \begin{enumerate}
%         \item limitations of the current model: effectiveness, efficiency, etc.
%         \item how to fine-tune a new model?
%         \item evaluate the performance of the fine-tuned model
%         \item ablation on different fine-tuning settings (w/, w/o questionnaire, resoning, DPO, SFT)
%     \end{enumerate}
% }

With previous experiments, we noticed several limitations of the current model, including effectiveness and efficiency. To address these limitations, we tried to align LLM to fit the BFI prediction task better.

\paragraph{Limitations of Current Model} The current model exhibits limitations in terms of effectiveness and efficiency. As shown in Tab.~\ref{tab:model_ablation}, with scale larger than 34B, the model could show statistically significant correlation. However, the efficiency of these models is a concern, as they require substantial computational resources. And with the largest and most powerful model, Qwen1.5-110B-Chat~\cite{bai2023qwen}, it only reach moderate correlation. In consideration of the specialized nature of the BFI prediction task, we sought to align the LLMs more closely with this task to enhance prediction validity.

\paragraph{Aligning LLMs} We choose Meta-Llama-3-8B-Instruct-BFI~\cite{llama3} as the base model for fine-tuning for its strong performance and suitable model size. Inspired by ~\citet{pang2024iterative}, We use DPO(Direct Preference Optimization)~\cite{rafailov2023direct} with SFT(Supervised Fine-Tuning) to align the model with the BFI prediction task. We extract generated responses from the models in ~\ref{tab:model_ablation} and select answers with minimum error to form the ``chosen'' selection for both DPO and SFT training and answers with maximum error to form the ``rejected'' selection for DPO training. The results are shown in Tab.~\ref{tab:model_ablation} and Fig.~\ref{fig:mae_analysis}, our fine-tuned model exhibits a significant improvement than original base model in prediction validity, and even outperforms the largest model Qwen1.5-110B-Chat~\cite{bai2023qwen}. In efficiency, Qwen1.5-110B-Chat requires 8 A100 GPUs at 2 requests per second, while our fine-tuned model can run with 1 A100 GPU at 6.87 requests per second.

We further study the impact of different fine-tuning settings. Limited by space, we report technical details and results in Sec.~\ref{sec:appendix:fine_tuning} in the appendix.


% \subsection{Results and Analysis}

% The outcomes of our experiments provide insightful answers to our research questions, demonstrating the nuanced capabilities of LLMs in predicting BFI traits from psycho-counseling dialogues.

% \subsubsection{RQ1: validity of LLM Predictions}
% We begin our analysis by examining the validity of LLM predictions in psycho-counseling dialogues. First, we test the baseline performance that directly predicts BFI traits from the dialogues and use Pearson correlation coefficient for criterion validity. The results are shown in Table.\ref{tab:correlation_no_questionnaire}, which shows a poor performance. This is consistent with Item Response Theory~\cite{baker2001basics,reise2009item,embretson2013item} that personality is complex and hard to be measured directly, so tools like client are needed.

% % \input{tables/correlation_no_questionnaire.tex}

% % With this in mind, we extend our simulations to using the questionnaire of client to guide the LLMs in predicting the BFI traits. As shown in Figure\ref{fig:correlation_roles}, "no-role" represents the baseline performance that directly predicts BFI traits from the dialogues with answering the questionnaire. Compared to Table\ref{tab:correlation_no_questionnaire}, the performance is significantly improved and "extraversion", "negative emotionality","open mindedness" have shown significant correlation.
% In pursuit of enhancing our understanding, we have broadened our simulations by incorporating the client questionnaire as a guiding tool for LLMs in predicting personality traits. As depicted in Figure\ref{fig:correlation_roles}, the baseline scenario, denoted as "no-role," directly derives BFI traits from dialogues without utilizing the questionnaire. The comparative analysis, as highlighted in Table\ref{tab:correlation_no_questionnaire}, reveals a marked enhancement in performance. Notably, traits such as "extraversion," "negative emotionality," and "open-mindedness" exhibit substantial correlations.

% % This encourages us to further explore using questionnaire. We extend our simulations to include the roles of psychological counseling, including the roles of client who fill the questionnaire by default, counselor who is interacting with the client in counseling, and observer who stands for observer rating in previous studies. For ``client'' and ``counselor'', counseling dialogue is used as the multi-turn chat history for LLM to predict the choice of questionnaire, for ``observer'', dialogue is used in single-turn. The results are shown in Figure\ref{fig:correlation_roles}, which shows that the validity of predictions is notably enhanced by role-play. The client role shows the strongest correlation, which is consistent with the principles of Item Response Theory~\cite{baker2001basics,reise2009item,embretson2013item} that direct responses of clients are the most reliable source of personality assessment information.
% This positive outcome encourages further exploration into the integration of questionnaires within our simulations. We have expanded our model to simulate the dynamics of psychological counseling by introducing distinct roles: the 'client' who completes the questionnaire, the 'counselor' who facilitates the session, and the 'observer' who represents external ratings found in prior studies. The 'client' and 'counselor' engage in multi-turn counseling dialogues, which serve as data for the LLM to predict responses to the questionnaire. For the 'observer,' the model processes dialogue in a single-turn format. The results, illustrated in Figure\ref{fig:correlation_roles}, demonstrate that role-play significantly boosts the validity of predictions. Consistent with the principles of Item Response Theory as outlined, the client's direct responses are identified as the most reliable indicators for personality assessment.

% We further employ different state-of-the-art LLMs, including Qwen1.5-72B-Chat~\cite{bai2023qwen}, Yi-34B-Chat~\cite{ai2024yi}, AquilaChat2-34B~\cite{Aquila2}, Baichuan2-13B-Chat~\cite{yang2023baichuan}, Gemma-1.1-7B-IT~\cite{gemmateam2024gemma}, and ChatGLM3-6B-128k~\cite{zeng2023glmb}, to evaluate the performance of different models in predicting the BFI traits. We also assess the reliability of these models using Cronbach's Alpha and Kappa statistics, as shown in Table\ref{tab:models_reliability}. The results indicate that Qwen1.5-72B-Chat~\cite{bai2023qwen} exhibits the highest reliability, with a Cronbach's Alpha of 0.857, followed by Yi-34B-Chat~\cite{ai2024yi} and ChatGLM3-6B-128k~\cite{zeng2023glmb}.

% Besides, the validity of different models is also tested. According to the Pearson correlation between predicted and actual BFI traits, Qwen1.5-72B-Chat~\cite{bai2023qwen}, Qwen-72B-Chat~\cite{bai2023qwen}, Yi-34B-Chat~\cite{ai2024yi} show strong and statistically significant correlation for all traits. The full results are shown in Figure \ref{fig:correlation_LLMs} in the appendix for space limitation.

% As Qwen1.5 is the best model in terms of validity and reliability, we perform the last but not least, a ablation study to see the impact of model size on the performance. Since model size is a key factor in the performance of LLMs, we test the performance of Qwen1.5 serires with different model sizes, including 0.5B, 1.8B, 4B, 7B, 14B, 72B. Results show that the performance is improved with the increase of model size, and with size greater than 4B, the performance is stable significantly. The results are shown in Figure\ref{fig:correlation-modelsize} in the appendix.

% % % Reliability
% % Our investigation into the validity of LLM predictions commenced with an assessment of reliability, utilizing Cronbach's Alpha and the Kappa statistic for test-retest reliability. The Cronbach's Alpha value of 0.847 signifies a high degree of internal consistency among the BFI traits as predicted by LLMs, suggesting that the models capture a coherent representation of personality traits that aligns well with the theoretical constructs of the Big Five. The Kappa statistic, marked as XXX, indicates strong test-retest reliability, affirming that the LLMs' predictions are stable over time and not significantly influenced by random fluctuations or the specificities of the dialogues.

% % % Validity
% % The validity of the LLM predictions was assessed through the Pearson correlation coefficient, with the baseline results depicted in Figure\ref{fig:experiments}. This analysis revealed a strong and statistically significant correlation for traits such as "Extraversion", "Conscientiousness", "Negative Emotionality", and "Open Mindedness", demonstrating the LLMs' capability to accurately predict these dimensions. "Agreeableness", however, exhibited a moderate correlation, echoing the challenges highlighted in previous studies XXX, which have identified "Agreeableness" as a particularly complex trait to predict accurately.

% \input{tables/models_reliability.tex}

% % Expanding the scope of our analysis, we examined the role-play performance of counselor and observer, alongside the client role, across different models including GPT-4 and Gemini-Ultra. The resulting Cronbach's Alpha values for these configurations were recorded as XXX and XXX, respectively, with corresponding Kappa statistics marked as XXX and XXX. These findings underscore the versatility and robustness of LLMs across various roles and models, indicating their potential for reliable personality trait prediction in diverse counseling scenarios.

% % For validity of different roles and models, summarized in Table.XXX, revealed that the "client" role achieved the highest correlation coefficients, followed by "Counselor" and "Observer". This hierarchy of predictive validity resonates with the principles of Item Response Theory, which posits the direct responses of clients as the most reliable source of personality assessment information. The "Counselor" role, representing an observer within the counseling session, and the "Observer" role, indicative of a third-party perspective, exhibited diminished validity in trait assessment, highlighting the inherent challenges in assessing personality traits from indirect observations.

% % For different models, To be updated...

% These results collectively affirm the potential of LLMs to serve as powerful tools in the non-intrusive prediction of BFI traits within psycho-counseling dialogues. The high reliability and notable validity across various roles and models underscore the sophistication of LLMs in understanding and interpreting complex human behaviors and emotional states. However, the nuanced performance across different traits and the varying effectiveness of roles and models also point to areas for further refinement and exploration in the quest to fully harness the capabilities of LLMs for psychological assessment.

% \subsubsection{RQ2: Impact of Dialogue Session Characteristics}

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=\linewidth]{figures/error_analysis_per_dimension.png}
%     \caption{Boxplot of error between predicted and actual BFI traits for each dimension and averaged over all dimensions. Red line indicates the $error=1$, which is the threshold of significant error.}
%     \label{fig:error_analysis_per_dimension}
% \end{figure}

% To perform a detailed analysis of validity, we examine the impact of different dialogue session characteristics on the validity of BFI Trait predictions. We first compute the absolute error between the predicted and actual BFI traits for each dimension, as shown in Figure\ref{fig:error_analysis_per_dimension}. We argue that an error greater than 1 is significant, because in client, the score of each question is from 1 to 5. if the error is greater than 1, it means a wrong prediction of the question. We average the error over all dimensions to get the overall error of the prediction, named as "average" in the figure.

% With Interquartile Range (IQR), outliers are identified as values that fall below Q1 - 1.5 * IQR or above Q3 + 1.5 * IQR as it shown in Figure\ref{fig:error_analysis_per_dimension}. It's important to analysis why LLMs make the wrong choice, so we perform 2 experiment to check content validity. The first is to analysis the error per question in session, we employ the most powerful LLM in reasoning, Gemini-Ultra~\cite{geminiteam2024gemini}, to generate the reason for the wrong choice by offering dialogue, question, predicted answer with reasoning and actual answer. We sample 10 outliers from each dimension with $error=4$, which means completely wrong prediction. The second is to compare the difference between the best and worst session per dimension. We take all outliers from each dimensions as the worst sessions, and sample the same number of sessions with the smallest error as the best sessions. We then feed the dialogue into Gemini-Ultra~\cite{geminiteam2024gemini} to analysis the reason for the difference.

% For the first experiment, we place LLM as "The third-party analyser" in prompt to feed to Gemini-Ultra and summarize all reasons together. The results show that shortcomings of LLM in predicting BFI traits from dialogues include:

% \noindent \textbf{Limited Context:} \textit{The dialogue records may only reflect the visitor's behavior and expressions in specific contexts, which may not fully reflect their performance in daily life.}\\
% \noindent \textbf{Bias of Third-party Perspective:} \textit{The interpretation of dialogue records by third-party analysts may be influenced by subjective factors such as personal values and cultural background.}\\
% \noindent \textbf{Lack of Background Information:} \textit{Third-party analysts usually cannot obtain visitors' personal growth experiences, family environment, and other background information, which may affect the accurate assessment of personality traits.}

% Meanwhile, Gemini-Ultra also finds and reports the reasons for the wrong choice in the sample outliers, which can be summarized as:

% \noindent \textbf{Self-awareness bias:} \textit{clients may have a certain bias in their self-perception, overestimating or underestimating certain aspects of their performance.}\\
% \noindent \textbf{Social Expectation Bias:} \textit{clients may tend to provide answers that meet social expectations, especially in psychological counseling or testing environments.}\\
% \noindent \textbf{Situational Factors:} \textit{clients' behavior and answers in different situations may differ, such as in counseling and in daily life.}

% We present the full response in Appendix due to space limitation.



% \subsubsection{RQ3:     }

% To answer RQ3, we extend

% % \begin{table}[t]
% %     \centering
% %     \resizebox{0.8\linewidth}{!}{
% %         \begin{tabular}{lrrrrrrr}
% %             \toprule
% %             Client ID & Session \# & Error \# & E \# & A \# & C  \# & N  \# & O  \# \\
% %             \midrule
% %             A223      & 10         & 9        & 0    & 6    & 1     & 0     & 10    \\
% %             A221      & 10         & 6        & 0    & 1    & 8     & 1     & 0     \\
% %             A254      & 10         & 6        & 0    & 0    & 0     & 9     & 2     \\
% %             A154      & 10         & 5        & 4    & 0    & 2     & 0     & 2     \\
% %             A025      & 10         & 5        & 0    & 0    & 0     & 0     & 1     \\
% %             A076      & 10         & 2        & 0    & 0    & 0     & 3     & 0     \\
% %             A237      & 10         & 2        & 0    & 0    & 0     & 0     & 1     \\
% %             A095      & 10         & 2        & 0    & 1    & 0     & 0     & 0     \\
% %             A207      & 10         & 2        & 0    & 2    & 1     & 1     & 0     \\
% %             A235      & 10         & 2        & 2    & 0    & 0     & 0     & 5     \\
% %             \bottomrule
% %         \end{tabular}
% %         % \caption{Top 10 of 25 clients with most outlier sessions}
% %     }
% % \end{table}


==> tables/correlation_no_questionnaire.tex <==
% \begin{table}[t]
%   \centering
%   \resizebox{\linewidth}{!}{
%     \begin{tabular}{llccccc}
%       \toprule
%       Type of Role-Play           &   & E       & A      & C      & N       & O      \\
%       \midrule
%       \multirow[t]{5}{*}{no-role} & E & 0.154   & 0.046  & 0.119  & -0.042  & 0.271* \\
%                                   & A & -0.075  & 0.040  & -0.206 & 0.306** & -0.067 \\
%                                   & A & 0.093   & 0.071  & 0.119  & -0.075  & 0.119  \\
%                                   & N & -0.166  & 0.013  & 0.027  & 0.179   & -0.152 \\
%                                   & O & -0.237* & -0.128 & -0.197 & 0.164   & -0.059 \\
%       % \midrule
%       % \multirow[t]{5}{*}{Client}  & E & 0.009   & 0.129  & 0.025  & -0.065  & -0.057 \\
%       %                             & A & 0.053   & 0.065  & -0.001 & -0.182  & -0.109 \\
%       %                             & C & 0.087   & 0.147  & 0.216  & -0.162  & 0.030  \\
%       %                             & N & -0.069  & -0.019 & -0.045 & 0.085   & -0.192 \\
%       %                             & O & 0.012   & -0.059 & -0.060 & 0.019   & -0.001 \\
%       \bottomrule
%     \end{tabular}
%   }
%   \caption{Pearson correlation coefficient between predicted and actual Big Five traits without questionnaires, with and without role-play. * indicates p-value < 0.05, ** indicates p-value < 0.01. "E", "A", "C", "N", and "O" represent "Extraversion", "Agreeableness", "Conscientiousness", "Negative Emotionality", and "Open Mindedness", respectively.}
%   \label{tab:correlation_no_questionnaire}
% \end{table}

==> tables/method_ablation.tex <==
% \begin{table*}[t]
%     \centering
%     \resizebox{\textwidth}{!}{
%         \begin{tabular}{lllllll}
%             % \toprule
%             %                                   & Mean Value & Open Mindedness & Conscientiousness & Extraversion  & Agreeableness & Negative Emotionality \\
%             %                                   &            &                 &                   &               &               &                       \\
%             % \midrule
%             % Baseline                          & 0.086      & 0.154           & 0.040             & 0.119         & 0.179         & -0.059                \\
%             % \em + Role-Play                   & 0.074      & 0.009           & 0.065             & 0.216         & 0.085         & -0.001                \\
%             % \em + Questionnaire               & 0.261      & 0.230$^*$       & 0.203             & 0.304$^{**}$  & 0.113         & 0.455$^{***}$         \\
%             % \em + Role-Play and Questionnaire & 0.472      & 0.491$^{***}$   & 0.449$^{***}$     & 0.542$^{***}$ & 0.350$^{**}$  & 0.531$^{***}$         \\
%             % \bottomrule
%             \toprule
%                                               & Open Mindedness & Conscientiousness & Extraversion & Agreeableness & Negative Emotionality & Avg.  \\
%             Role                              &                 &                   &              &               &                       &       \\
%             \midrule
%             no-role                           & 0.216           & 0.264*            & 0.272*       & 0.028         & 0.237*                & 0.203 \\
%             \em + Role-Play                   & 0.241*          & 0.012             & -0.068       & -0.126        & -0.060                & 0.000 \\
%             \em + Questionnaire               & 0.263*          & 0.281*            & 0.482***     & 0.077         & 0.317**               & 0.284 \\

%             \em + Role-Play and Questionnaire & 0.457***        & 0.480***          & 0.562***     & 0.412***      & 0.561***              & 0.494 \\
%             \bottomrule
%         \end{tabular}
%     }
%     \caption{ Baseline is the naive prediction without any strategy. The results reported for \textit{Role-play} is from the role \textit{client} . * p-value < 0.05, ** p-value < 0.01, *** p-value < 0.001. \YY{TODO: 1. Add name for the table. 2. Update description for clear understanding. 3. Update data with the latest results.}}
%     \label{tab:method_ablation}
% \end{table*}

% \begin{table*}
%     \centering
%     \resizebox{\textwidth}{!}{
%         \begin{tabular}{llllllr}
%             \toprule
%                                               & Open Mindedness   & Conscientiousness  & Extraversion      & Agreeableness     & Negative Emotionality & Avg.           \\
%             Method                            &                   &                    &                   &                   &                       &                \\
%             \midrule
%             Baseline                          & 0.019             & 0.146              & 0.110             & 0.161             & -0.118                & 0.064          \\
%             \em + Role-Play                   & 0.024             & -0.073             & 0.003             & 0.020             & 0.297*                & 0.054          \\
%             \em + Questionnaire               & 0.455***          & 0.455***           & 0.421***          & 0.230             & 0.515***              & 0.415          \\
%             \em + Role-Play and Questionnaire & \textbf{0.692***} & \textbf{0.554*** } & \textbf{0.569***} & \textbf{0.448***} & \textbf{0.648***}     & \textbf{0.582} \\
%             % \cline{1-8}
%             \bottomrule
%         \end{tabular}
%     }
%     \caption{Correlation of predicted BFI traits with the ground truth. We compare the direct prediction of BFI traits using LLMs with adding role-play, questionnaire, and a combination of both. The findings show that combining role-play and questionnaire-based prompts significantly enhances prediction accuracy in most traits. Interestingly, the role-play method alone does not offer any improvement, underscoring the value of structured input from questionnaires with psychology priori in boosting model performance. * indicates p-value < 0.05, ** indicates p-value < 0.01, *** indicates p-value < 0.001.}
%     \label{tab:method_ablation}
% \end{table*}

\begin{table*}[t]
    \centering
    \resizebox{\textwidth}{!}{
        \begin{tabular}{lllllllr}
            \toprule
                                                                  &                              & Open Mindedness & Conscientiousness & Extraversion & Agreeableness & Negative Emotionality & Avg.   \\
            Method                                                & Model                        &                 &                   &              &               &                       &        \\
            \midrule

            \multirow[t]{3}{*}{Baseline}                          & Meta-Llama-3-8B-Instruct-BFI & 0.019           & 0.146             & 0.110        & 0.161         & -0.118                & 0.064  \\
                                                                  & Qwen1.5-110B-Chat            & 0.275*          & 0.141             & 0.347**      & 0.122         & 0.356**               & 0.248  \\
                                                                  & Avg.                         & 0.147           & 0.144             & 0.229        & 0.142         & 0.119                 & 0.156  \\
            \cline{1-8}
            \multirow[t]{3}{*}{\em + Role-Play Only}              & Meta-Llama-3-8B-Instruct-BFI & 0.024           & -0.073            & 0.003        & 0.020         & 0.297*                & 0.054  \\
                                                                  & Qwen1.5-110B-Chat            & -0.113          & 0.020             & -0.130       & 0.011         & 0.128                 & -0.017 \\
                                                                  & Avg.                         & -0.044          & -0.026            & -0.063       & 0.015         & 0.212                 & 0.019  \\
            \cline{1-8}
            \multirow[t]{3}{*}{\em + Questionnaire Only}          & Meta-Llama-3-8B-Instruct-BFI & 0.455***        & 0.455***          & 0.421***     & 0.230         & 0.515***              & 0.415  \\
                                                                  & Qwen1.5-110B-Chat            & 0.183           & 0.236*            & 0.409***     & 0.090         & 0.349**               & 0.253  \\
                                                                  & Avg.                         & 0.319           & 0.345             & 0.415        & 0.160         & 0.432                 & 0.334  \\
            \cline{1-8}
            \multirow[t]{3}{*}{\em + Role-Play and Questionnaire} & Meta-Llama-3-8B-Instruct-BFI & 0.692***        & 0.554***          & 0.569***     & 0.448***      & 0.648***              & 0.582  \\
                                                                  & Qwen1.5-110B-Chat            & 0.457***        & 0.480***          & 0.562***     & 0.412***      & 0.561***              & 0.495  \\
                                                                  & Avg.                         & 0.574           & 0.517             & 0.566        & 0.430         & 0.605                 & 0.538  \\
            % \cline{1-8}
            \bottomrule
        \end{tabular}
    }
    \caption{Comparison of Different Methods for Predicting BFI Traits. We evaluated the direct prediction of BFI traits using LLMs and compared it with adding a role-play, questionnaire, and a combination of both. The findings show that the combination of role-play and questionnaire-based prompts significantly enhances prediction accuracy, with Meta-Llama-3-8B-Instruct-BFI (Ours) outperforming Qwen1.5-110B-Chat~\cite{bai2023qwen} in most traits. Interestingly, the role-play method alone does not offer any improvement, underscoring the value of structured input from questionnaires with psychology priori in boosting model performance.}
    \label{tab:method_ablation}
\end{table*}

==> tables/model_ablation.tex <==
\begin{table*}[t]
    \centering
    \resizebox{\linewidth}{!}{
        % \begin{tabular}{llllll}
        %     \toprule
        %                                                & extraversion & agreeableness & conscientiousness & negative emotionality & open mindedness \\
        %     model\_name                                &              &               &                   &                       &                 \\
        %     \midrule
        %     Qwen1.5-72B-Chat~\cite{bai2023qwen}        & 0.542***     & 0.350**       & 0.449***          & 0.531***              & 0.491***        \\
        %     Qwen-72B-Chat~\cite{bai2023qwen}           & 0.510***     & 0.400***      & 0.470***          & 0.516***              & 0.480***        \\
        %     Meta-Llama-3-70B-Instruct~\cite{llama3}    & 0.373**      & 0.380**       & 0.434***          & 0.282*                & 0.391***        \\
        %     Yi-34B-Chat~\cite{ai2024yi}                & 0.544***     & 0.324**       & 0.440***          & 0.350**               & 0.456***        \\
        %     AquilaChat2-34B~\cite{Aquila2}             & 0.188        & 0.022         & 0.119             & 0.206                 & 0.110           \\
        %     Baichuan2-13B-Chat~\cite{yang2023baichuan} & 0.029        & 0.070         & -0.044            & 0.237*                & 0.059           \\
        %     % Meta-Llama-3-8B-Instruct~\cite{llama3} & 0.233 & 0.111 & 0.434*** & 0.303* & 0.177 \\
        %     gemma-1.1-7b-it~\cite{gemmateam2024gemma}  & 0.329**      & 0.037         & 0.169             & 0.070                 & 0.125           \\
        %     chatglm3-6b-128k~\cite{zeng2023glmb}       & -0.145       & -0.007        & -0.005            & 0.049                 & -0.039          \\
        %     \bottomrule
        % \end{tabular}
        % \begin{tabular}{llllll}
        % \toprule
        %                                            & Open Mindedness & Conscientiousness & Extraversion & Agreeableness & Negative Emotionality \\
        % Model Name                                 &                 &                   &              &               &                       \\
        % \midrule
        % gemini-1.5-pro-latest                      & 0.521***        & 0.438***          & 0.494***     & 0.356**       & 0.314**               \\
        % \midrule
        % Qwen1.5-110B-Chat                          & 0.457***        & 0.480***          & 0.562***     & 0.412***      & 0.561***              \\
        % Qwen1.5-72B-Chat~\cite{bai2023qwen}        & 0.491***        & 0.449***          & 0.542***     & 0.350**       & 0.531***              \\
        % Qwen-72B-Chat~\cite{bai2023qwen}           & 0.480***        & 0.470***          & 0.510***     & 0.400***      & 0.516***              \\
        % Meta-Llama-3-70B-Instruct~\cite{llama3}    & 0.391***        & 0.434***          & 0.373**      & 0.380**       & 0.282*                \\
        % Yi-34B-Chat~\cite{ai2024yi}                & 0.456***        & 0.440***          & 0.544***     & 0.324**       & 0.350**               \\
        % AquilaChat2-34B~\cite{Aquila2}             & 0.110           & 0.119             & 0.188        & 0.022         & 0.206                 \\
        % internlm2-chat-20b~\cite{cai2024internlm2} & 0.240*          & 0.345**           & 0.434***     & 0.221         & 0.206                 \\
        % Baichuan2-13B-Chat~\cite{yang2023baichuan} & 0.059           & -0.044            & 0.029        & 0.070         & 0.237*                \\
        % % Meta-Llama-3-8B-Instruct & 0.177 & 0.434*** & 0.233 & 0.111 & 0.303* \\
        % gemma-1.1-7b-it~\cite{gemmateam2024gemma}  & 0.125           & 0.169             & 0.329**      & 0.037         & 0.070                 \\
        % chatglm3-6b-128k~\cite{zeng2023glmb}       & -0.039          & -0.005            & -0.145       & -0.007        & 0.049                 \\
        % \bottomrule
        \begin{tabular}{llllllr}
            \toprule
                                                                & Open Mindedness   & Conscientiousness & Extraversion      & Agreeableness     & Negative Emotionality & Avg.           \\
            Model                                               &                   &                   &                   &                   &                       &                \\
            \midrule
            GPT-4-turbo~\cite{openai2023gpt4}                   & 0.407***          & 0.360**           & 0.507***          & 0.303*            & 0.337**               & 0.383          \\
            gemini-1.5-pro-latest~\cite{geminiteam2024gemini}   & 0.521***          & 0.438***          & 0.494***          & 0.356**           & 0.314**               & 0.425          \\
            gemini-1.5-flash-latest~\cite{geminiteam2024gemini} & 0.304*            & 0.357**           & 0.248*            & 0.358**           & 0.320**               & 0.317          \\
            gemini-1.0-ultra-latest~\cite{geminiteam2024gemini} & 0.412***          & 0.316**           & 0.372**           & 0.057             & 0.309*                & 0.293          \\
            gemini-1.0-pro-001~\cite{geminiteam2024gemini}      & 0.366**           & 0.309*            & 0.320**           & 0.117             & 0.294*                & 0.281          \\
            qwen-long~\cite{bai2023qwen}                        & 0.346**           & 0.376**           & 0.451***          & 0.265*            & 0.405***              & 0.369          \\
            qwen-turbo~\cite{bai2023qwen}                       & 0.363**           & 0.314**           & 0.418***          & 0.279*            & 0.321**               & 0.339          \\
            ERNIE-Speed-128K~\cite{ernie}                       & 0.138             & 0.167             & 0.241*            & -0.203            & 0.239*                & 0.116          \\
            ERNIE-Lite-8K-0308~\cite{ernie}                     & -0.118            & -0.030            & 0.148             & -0.237            & 0.285*                & 0.010          \\
            \midrule
            Qwen1.5-110B-Chat~\cite{bai2023qwen}                & 0.457***          & 0.480***          & 0.562***          & 0.412***          & 0.561***              & 0.494          \\
            % Qwen1.5-72B-Chat                                       & 0.491***        & 0.449***          & 0.542***     & 0.350**       & 0.531***              & 0.473  \\
            Qwen-72B-Chat~\cite{bai2023qwen}                    & 0.480***          & 0.470***          & 0.510***          & 0.400***          & 0.516***              & 0.475          \\
            Meta-Llama-3-70B-Instruct~\cite{llama3}             & 0.368***          & 0.497***          & 0.492***          & 0.375***          & 0.369***              & 0.420          \\
            deepseek-llm-67b-chat~\cite{deepseekai2024deepseek} & 0.312**           & 0.412***          & 0.476***          & 0.301**           & 0.444***              & 0.389          \\
            Yi-1.5-34B-Chat~\cite{ai2024yi}                     & 0.350**           & 0.369***          & 0.451***          & 0.242*            & 0.328**               & 0.348          \\
            Yi-34B-Chat~\cite{ai2024yi}                         & 0.456***          & 0.440***          & 0.544***          & 0.324**           & 0.350**               & 0.423          \\
            AquilaChat2-34B        \cite{Aquila2}               & 0.110             & 0.119             & 0.188             & 0.022             & 0.206                 & 0.129          \\
            internlm2-chat-20b     \cite{cai2024internlm2}      & 0.240*            & 0.345**           & 0.434***          & 0.221             & 0.206                 & 0.289          \\
            Baichuan2-13B-Chat~\cite{yang2023baichuan}          & 0.059             & -0.044            & 0.029             & 0.070             & 0.237*                & 0.070          \\
            glm-4-9b-chat~\cite{zeng2023glmb}                   & 0.293*            & 0.312**           & 0.240*            & 0.036             & 0.305*                & 0.237          \\
            gemma-1.1-7b-it~\cite{gemmateam2024gemma}           & 0.125             & 0.169             & 0.329**           & 0.037             & 0.070                 & 0.146          \\
            % chatglm3-6b-128k~\cite{zeng2023glmb}                & -0.039            & -0.005            & -0.145            & -0.007            & 0.049                 & -0.029         \\
            % % \bottomrule
            % Qwen1.5-72B-Chat~\cite{bai2023qwen}        & 0.857             & 0.063 & 1          \\
            % Qwen-72B-Chat~\cite{bai2023qwen}           & 0.781             & 0.039 & 1          \\
            % Yi-34B-Chat~\cite{ai2024yi}                & 0.825             & 0.029 & 1          \\
            % AquilaChat2-34B~\cite{Aquila2}             & 0.400             & 0.010 & 1          \\
            % Baichuan2-13B-Chat~\cite{yang2023baichuan} & 0.791             & 0.008 & 1          \\
            % gemma-1.1-7b-it~\cite{gemmateam2024gemma}  & 0.903             & 0.016 & 1          \\
            % chatglm3-6b-128k~\cite{zeng2023glmb}       & 0.818             & 0.009 & 1          \\
            \midrule
            Meta-Llama-3-8B-Instruct~\cite{llama3}              & 0.177             & 0.434***          & 0.233             & 0.111             & 0.303*                & 0.252          \\
            % Meta-Llama-3-8B-Instruct-BFI-anonymous (Ours)          & 0.463***        & 0.409***          & 0.456***     & 0.429***      & 0.548***              & 0.461  \\
            % Meta-Llama-3-8B-Instruct-BFI                           & 0.636***        & 0.514***          & 0.570***     & 0.182         & 0.612***              & 0.503  \\
            Meta-Llama-3-8B-Instruct-BFI (Ours)                 & \textbf{0.692***} & \textbf{0.554***} & \textbf{0.569***} & \textbf{0.448***} & \textbf{0.648***}     & \textbf{0.582} \\
            % Meta-Llama-3-8B-Instruct-BFI(Ours-AI Cluster) & 0.660*** & 0.425*** & 0.522*** & 0.281* & 0.528*** & 0.483 \\

            % Meta-Llama-3-8B-Instruct-BFI-ckpt-3250 & 0.696***        & 0.526***          & 0.624***     & 0.426***      & 0.676***              & 0.590  \\
            % Meta-Llama-3-8B-Instruct-BFI-ckpt-3000 & 0.676***        & 0.630***          & 0.606***     & 0.372**       & 0.653***              & 0.587  \\
            % Meta-Llama-3-8B-Instruct-BFI-ckpt-2750 & 0.714***        & 0.542***          & 0.655***     & 0.307*        & 0.589***              & 0.561  \\
            % Meta-Llama-3-8B-Instruct-BFI-ckpt-2500 & 0.589***        & 0.555***          & 0.601***     & 0.350**       & 0.603***              & 0.540  \\
            % Meta-Llama-3-8B-Instruct-BFI-ckpt-2250 & 0.641***        & 0.552***          & 0.517***     & 0.449***      & 0.588***              & 0.549  \\
            % Meta-Llama-3-8B-Instruct-BFI-ckpt-2000 & 0.673***        & 0.506***          & 0.466***     & 0.235         & 0.645***              & 0.505  \\
            % Meta-Llama-3-8B-Instruct-BFI-ckpt-1750 & 0.579***        & 0.352**           & 0.541***     & 0.375**       & 0.566***              & 0.483  \\
            % Meta-Llama-3-8B-Instruct-BFI-ckpt-1500 & 0.500***        & 0.493***          & 0.417***     & 0.442***      & 0.626***              & 0.496  \\
            % Meta-Llama-3-8B-Instruct-BFI-ckpt-1250 & 0.557***        & 0.564***          & 0.491***     & 0.217         & 0.502***              & 0.466  \\
            % Meta-Llama-3-8B-Instruct-BFI-ckpt-1000 & 0.446***        & 0.351**           & 0.478***     & 0.191         & 0.361**               & 0.365  \\
            % Meta-Llama-3-8B-Instruct-BFI-ckpt-750  & 0.447***        & 0.449***          & 0.351**      & 0.300*        & 0.341**               & 0.378  \\
            % Meta-Llama-3-8B-Instruct-BFI-ckpt-500  & 0.467***        & 0.347**           & 0.531***     & 0.306*        & 0.125                 & 0.355  \\
            % Meta-Llama-3-8B-Instruct-BFI-ckpt-250  & 0.417***        & 0.470***          & 0.371**      & 0.235         & 0.116                 & 0.322  \\
            \bottomrule
        \end{tabular}
    }
    \caption{Correlation of Predicted and Actual BFI Traits across Various Large Language Models. The models include state-of-the-art proprietary model such as GPT-4, gemini, and several open-sourced model such as Llama3, Qwen, Yi, etc. The results highlight the variability in predictive validity across models, with certain models, particularly the fine-tuned Meta-Llama-3-8B-Instruct-BFI (ours) models, showing notably higher correlation coefficients, demonstrates the highest overall performance, underscoring the efficacy of our tailored fine-tuning approach. Significance levels are denoted by * (p-value < 0.05), ** (p-value < 0.01), and *** (p-value < 0.001), indicating robust statistical support for the correlations observed.
    }
    \label{tab:model_ablation}

\end{table*}


% \begin{table*}
%     \centering
%     \resizebox{\textwidth}{!}{
%         % \begin{tabular}{lr|lllllr}
%         %     \toprule
%         %      & Cronbach $\alpha$ & Open Mindedness & Conscientiousness & Extraversion & Agreeableness & Negative Emotionality & Avg. \\
%         %     Model &  &  &  &  &  &  &  \\
%         %     \midrule
%         %     GPT-4-turbo~\cite{openai2023gpt4} & 0.731 & 0.370** & 0.318** & 0.493*** & 0.248* & 0.312** & 0.348 \\
%         %     gemini-1.5-pro-latest~\cite{geminiteam2024gemini} & 0.802 & 0.521*** & 0.438*** & 0.494*** & 0.356** & 0.314** & 0.425 \\
%         %     gemini-1.5-flash-latest~\cite{geminiteam2024gemini} & 0.888 & 0.304* & 0.357** & 0.248* & 0.358** & 0.320** & 0.317 \\
%         %     gemini-1.0-ultra-latest~\cite{geminiteam2024gemini} & 0.786 & 0.412*** & 0.316** & 0.372** & 0.057 & 0.309* & 0.293 \\
%         %     gemini-1.0-pro-001~\cite{geminiteam2024gemini} & 0.839 & 0.366** & 0.309* & 0.320** & 0.117 & 0.294* & 0.281 \\
%         %     qwen-long~\cite{bai2023qwen} & 0.848 & 0.346** & 0.376** & 0.451*** & 0.265* & 0.405*** & 0.369 \\
%         %     qwen-turbo~\cite{bai2023qwen} & 0.896 & 0.363** & 0.314** & 0.418*** & 0.279* & 0.321** & 0.339 \\
%         %     ERNIE-Speed-128K~\cite{ernie} & 0.864 & 0.138 & 0.167 & 0.241* & -0.203 & 0.239* & 0.116 \\
%         %     ERNIE-Lite-8K-0308~\cite{ernie} & 0.636 & -0.130 & -0.029 & 0.148 & -0.236 & 0.272* & 0.005 \\
%         %     \midrule
%         %     Qwen1.5-110B-Chat~\cite{bai2023qwen} & 0.830 & 0.457*** & 0.480*** & 0.562*** & 0.412*** & 0.561*** & 0.494 \\
%         %     Qwen-72B-Chat~\cite{bai2023qwen} & 0.781 & 0.480*** & 0.470*** & 0.510*** & 0.400*** & 0.516*** & 0.475 \\
%         %     Meta-Llama-3-70B-Instruct~\cite{llama3} & 0.841 & 0.368*** & 0.497*** & 0.492*** & 0.375*** & 0.369*** & 0.420 \\
%         %     deepseek-llm-67b-chat~\cite{deepseekai2024deepseek} & 0.635 & 0.312** & 0.412*** & 0.476*** & 0.301** & 0.444*** & 0.389 \\
%         %     Yi-1.5-34B-Chat~\cite{ai2024yi} & 0.846 & 0.350** & 0.369*** & 0.451*** & 0.242* & 0.328** & 0.348 \\
%         %     Yi-34B-Chat~\cite{ai2024yi} & 0.825 & 0.456*** & 0.440*** & 0.544*** & 0.324** & 0.350** & 0.423 \\
%         %     AquilaChat2-34B~\cite{Aquila2} & 0.400 & 0.110 & 0.119 & 0.188 & 0.022 & 0.206 & 0.129 \\
%         %     internlm2-chat-20b~\cite{cai2024internlm2} & 0.709 & 0.301** & 0.392*** & 0.427*** & 0.239* & 0.439*** & 0.360 \\
%         %     Baichuan2-13B-Chat~\cite{yang2023baichuan} & 0.791 & 0.059 & -0.044 & 0.029 & 0.070 & 0.237* & 0.070 \\
%         %     gemma-1.1-7b-it~\cite{gemmateam2024gemma} & 0.903 & 0.125 & 0.169 & 0.329** & 0.037 & 0.070 & 0.146 \\
%         %     chatglm3-6b-128k~\cite{zeng2023glmb} & 0.818 & -0.039 & -0.005 & -0.145 & -0.007 & 0.049 & -0.029 \\
%         %     % \midrule
%         %     Meta-Llama-3-8B-Instruct~\cite{llama3} & 0.908 & 0.177 & 0.434*** & 0.233 & 0.111 & 0.303* & 0.252 \\
%         %     Meta-Llama-3-8B-Instruct-BFI(Ours) & 0.711 & 0.692*** & 0.554*** & 0.569*** & 0.448*** & 0.648*** & 0.582 \\
%         %     Meta-Llama-3-8B-Instruct-BFI-anonymous(Ours) & 0.677 & 0.463*** & 0.409*** & 0.456*** & 0.429*** & 0.548*** & 0.461 \\
%         %     \bottomrule
%         %     \end{tabular}
%         \begin{tabular}{lr|lllllr}
%             \toprule
%              & Cronbach $\alpha$ & Open Mindedness & Conscientiousness & Extraversion & Agreeableness & Negative Emotionality & Avg. \\
%             Model &  &  &  &  &  &  &  \\
%             \midrule
%             GPT-4-turbo~\cite{openai2023gpt4} & 0.730 & 0.377** & 0.320** & 0.492*** & 0.258* & 0.312** & 0.352 \\
%             gemini-1.5-pro-latest~\cite{geminiteam2024gemini} & 0.802 & 0.521*** & 0.438*** & 0.494*** & 0.356** & 0.314** & 0.425 \\
%             gemini-1.5-flash-latest~\cite{geminiteam2024gemini} & 0.888 & 0.304* & 0.357** & 0.248* & 0.358** & 0.320** & 0.317 \\
%             gemini-1.0-ultra-latest~\cite{geminiteam2024gemini} & 0.786 & 0.412*** & 0.316** & 0.372** & 0.057 & 0.309* & 0.293 \\
%             gemini-1.0-pro-001~\cite{geminiteam2024gemini} & 0.839 & 0.366** & 0.309* & 0.320** & 0.117 & 0.294* & 0.281 \\
%             qwen-long~\cite{bai2023qwen} & 0.848 & 0.346** & 0.376** & 0.451*** & 0.265* & 0.405*** & 0.369 \\
%             qwen-turbo~\cite{bai2023qwen} & 0.896 & 0.363** & 0.314** & 0.418*** & 0.279* & 0.321** & 0.339 \\
%             ERNIE-Speed-128K~\cite{ernie} & 0.864 & 0.138 & 0.167 & 0.241* & -0.203 & 0.239* & 0.116 \\
%             ERNIE-Lite-8K-0308~\cite{ernie} & 0.636 & -0.130 & -0.029 & 0.148 & -0.236 & 0.272* & 0.005 \\
%             \midrule
%             Qwen1.5-110B-Chat~\cite{bai2023qwen} & 0.830 & 0.455*** & 0.463*** & 0.521*** & 0.334** & 0.354** & 0.425 \\
%             Qwen-72B-Chat~\cite{bai2023qwen} & 0.781 & 0.375** & 0.443*** & 0.391*** & 0.342** & 0.414*** & 0.393 \\
%             Meta-Llama-3-70B-Instruct~\cite{llama3} & 0.841 & 0.397*** & 0.467*** & 0.395*** & 0.284* & 0.289* & 0.366 \\
%             deepseek-llm-67b-chat~\cite{deepseekai2024deepseek} & 0.635 & 0.303* & 0.336** & 0.491*** & 0.196 & 0.301* & 0.325 \\
%             Yi-1.5-34B-Chat~\cite{ai2024yi} & 0.846 & 0.408** & 0.295* & 0.406** & 0.241 & 0.275* & 0.325 \\
%             Yi-34B-Chat~\cite{ai2024yi} & 0.825 & 0.399*** & 0.243* & 0.448*** & 0.297* & 0.204 & 0.318 \\
%             AquilaChat2-34B~\cite{Aquila2} & 0.400 & 0.085 & -0.059 & 0.126 & 0.035 & 0.248* & 0.087 \\
%             internlm2-chat-20b~\cite{cai2024internlm2} & 0.709 & 0.341** & 0.201 & 0.368** & 0.260* & 0.255* & 0.285 \\
%             Baichuan2-13B-Chat~\cite{yang2023baichuan} & 0.791 & -0.016 & 0.207 & 0.199 & 0.148 & -0.114 & 0.085 \\
%             gemma-1.1-7b-it~\cite{gemmateam2024gemma} & 0.903 & 0.054 & 0.330** & 0.364** & -0.053 & 0.034 & 0.146 \\
%             chatglm3-6b-128k~\cite{zeng2023glmb} & 0.818 & 0.057 & 0.054 & 0.005 & 0.062 & 0.011 & 0.038 \\
%             \midrule
%             Meta-Llama-3-8B-Instruct~\cite{llama3} & 0.908 & 0.177 & 0.434*** & 0.233 & 0.111 & 0.303* & 0.252 \\
%             Meta-Llama-3-8B-Instruct-BFI-anonymous(Ours) & 0.677 & 0.463*** & 0.409*** & 0.456*** & 0.429*** & 0.548*** & 0.461 \\
%             Meta-Llama-3-8B-Instruct-BFI(Ours) & 0.711 & 0.692*** & 0.554*** & 0.569*** & 0.448*** & 0.648*** & 0.582 \\
%             \bottomrule
%             \end{tabular}
%     }

% \label{tab:model_ablation}
% \end{table*}

==> tables/models_reliability.tex <==
% \begin{table}
%     \centering
%     \resizebox{\linewidth}{!}{
%         \begin{tabular}{lccc}
%             \toprule
%             Model Name                                 & Cronbach $\alpha$ & Kappa & Perplexity \\
%             \midrule
%             Qwen1.5-72B-Chat~\cite{bai2023qwen}        & 0.857             & 0.063 & 1          \\
%             Qwen-72B-Chat~\cite{bai2023qwen}           & 0.781             & 0.039 & 1          \\
%             Yi-34B-Chat~\cite{ai2024yi}                & 0.825             & 0.029 & 1          \\
%             AquilaChat2-34B~\cite{Aquila2}             & 0.400             & 0.010 & 1          \\
%             Baichuan2-13B-Chat~\cite{yang2023baichuan} & 0.791             & 0.008 & 1          \\
%             gemma-1.1-7b-it~\cite{gemmateam2024gemma}  & 0.903             & 0.016 & 1          \\
%             chatglm3-6b-128k~\cite{zeng2023glmb}       & 0.818             & 0.009 & 1          \\
%             \bottomrule
%         \end{tabular}
%     }
%     \caption{Cronbach's $\alpha$ and Kappa statistics for different LLMs in predicting Big Five Personality Traits. We use Qwen1.5-72B-Chat for its high reliability performance.}
%     \label{tab:models_reliability}
% \end{table}

==> tables/role_ablation.tex <==
% \begin{table*}
%     \centering
%     \resizebox{0.9\textwidth}{!}{
%         % \begin{tabular}{cllllllr}
%         %     \toprule
%         %                             &           & Open Mindedness & Conscientiousness & Extraversion & Agreeableness & Negative Emotionality & Avg.  \\
%         %     Turn Type               & Role Tpye &                 &                   &              &               &                       &       \\
%         %     % & Type of Role-Play &                 &                   &              &               &                       &       \\
%         %     \midrule
%         %     % No-Role           & 0.230*          & 0.203             & 0.304**      & 0.113         & 0.455***              \\
%         %     % \midrule
%         %     % Observer          & 0.317**         & 0.389***          & 0.350**      & 0.217         & 0.543***              \\
%         %     % Counselor         & 0.344**         & 0.255*            & 0.463***     & 0.163         & 0.505***              \\
%         %     % Client            & 0.491***        & 0.449***          & 0.542***     & 0.350**       & 0.531***              \\

%         %     % \multirow{4}{*}{single} & $\text{no-role}_{\text{single turn}}$   & 0.263*          & 0.281*            & 0.482***     & 0.077         & 0.317**               & 0.284 \\
%         %     %                              & $\text{observer}_{\text{single turn}}$  & 0.367***        & 0.435***          & 0.451***     & 0.306**       & 0.523***              & 0.416 \\
%         %     % % \midrule
%         %     % % && \cline{3-8}
%         %     %                              & $\text{client}_{\text{single turn}}$    & 0.407***        & 0.428***          & 0.503***     & 0.307**       & 0.507***              & 0.430 \\
%         %     %                              & $\text{counselor}_{\text{single turn}}$ & 0.426***        & 0.419***          & 0.501***     & 0.363***      & 0.566***              & 0.455 \\
%         %     \multirow{4}{*}{single} & client    & 0.407***        & 0.428***          & 0.503***     & 0.307**       & 0.507***              & 0.430 \\
%         %                             & counselor & 0.426***        & 0.419***          & 0.501***     & 0.363***      & 0.566***              & 0.455 \\
%         %                             & observer  & 0.367***        & 0.435***          & 0.451***     & 0.306**       & 0.523***              & 0.416 \\
%         %                             & no-role   & 0.263*          & 0.281*            & 0.482***     & 0.077         & 0.317**               & 0.284 \\
%         %     % \midrule
%         %     % && \cline{3-8}
%         %     \midrule
%         %     \multirow{2}{*}{multi}  & client    & 0.457***        & 0.480***          & 0.562***     & 0.412***      & 0.561***              & 0.494 \\
%         %                             & counselor & 0.332**         & 0.303**           & 0.478***     & 0.156         & 0.552***              & 0.364 \\

%         %     \bottomrule
%         % \end{tabular}
%         \begin{tabular}{llllllr}
%             \toprule
%                       & Open Mindedness   & Conscientiousness & Extraversion      & Agreeableness     & Negative Emotionality & Avg.           \\
%             Role      &                   &                   &                   &                   &                       &                \\
%             \midrule
%             no-role   & 0.455***          & 0.455***          & 0.421***          & 0.230             & 0.515***              & 0.415          \\
%             observer  & 0.499***          & 0.560***          & 0.476***          & 0.357**           & 0.483***              & 0.475          \\
%             counselor & 0.652***          & \textbf{0.586***} & 0.550***          & 0.412***          & 0.539***              & 0.548          \\
%             client    & \textbf{0.692***} & 0.554***          & \textbf{0.569***} & \textbf{0.448***} & \textbf{0.648***}     & \textbf{0.582} \\
%             \bottomrule
%         \end{tabular}
%     }
%     \caption{Performance of Models in Predicting BFI Traits Across Different Roles. We assess the predicting of BFI traits across various roles (client, counselor, observer, and no-role) in real-world counseling sessions. Our model consistently surpasses Qwen1.5-110B-Chat~\cite{bai2023qwen}, particularly in the client role, where it achieves the highest average correlation. This underscores the effectiveness of role-based prompting strategies, with the client and counselor roles showing significantly higher prediction accuracies. The no-role condition exhibits the lowest performance, emphasizing the importance of contextual role-play in improving model predictions. * indicates p-value < 0.05, ** indicates p-value < 0.01, *** indicates p-value < 0.001.}
%     \label{tab:role_ablation}
% \end{table*}

\begin{table*}[t]
    \centering
    \resizebox{\textwidth}{!}{
        % \begin{tabular}{cllllllr}
        %     \toprule
        %                             &           & Open Mindedness & Conscientiousness & Extraversion & Agreeableness & Negative Emotionality & Avg.  \\
        %     Turn Type               & Role Tpye &                 &                   &              &               &                       &       \\
        %     % & Type of Role-Play &                 &                   &              &               &                       &       \\
        %     \midrule
        %     % No-Role           & 0.230*          & 0.203             & 0.304**      & 0.113         & 0.455***              \\
        %     % \midrule
        %     % Observer          & 0.317**         & 0.389***          & 0.350**      & 0.217         & 0.543***              \\
        %     % Counselor         & 0.344**         & 0.255*            & 0.463***     & 0.163         & 0.505***              \\
        %     % Client            & 0.491***        & 0.449***          & 0.542***     & 0.350**       & 0.531***              \\

        %     % \multirow{4}{*}{single} & $\text{no-role}_{\text{single turn}}$   & 0.263*          & 0.281*            & 0.482***     & 0.077         & 0.317**               & 0.284 \\
        %     %                              & $\text{observer}_{\text{single turn}}$  & 0.367***        & 0.435***          & 0.451***     & 0.306**       & 0.523***              & 0.416 \\
        %     % % \midrule
        %     % % && \cline{3-8}
        %     %                              & $\text{client}_{\text{single turn}}$    & 0.407***        & 0.428***          & 0.503***     & 0.307**       & 0.507***              & 0.430 \\
        %     %                              & $\text{counselor}_{\text{single turn}}$ & 0.426***        & 0.419***          & 0.501***     & 0.363***      & 0.566***              & 0.455 \\
        %     \multirow{4}{*}{single} & client    & 0.407***        & 0.428***          & 0.503***     & 0.307**       & 0.507***              & 0.430 \\
        %                             & counselor & 0.426***        & 0.419***          & 0.501***     & 0.363***      & 0.566***              & 0.455 \\
        %                             & observer  & 0.367***        & 0.435***          & 0.451***     & 0.306**       & 0.523***              & 0.416 \\
        %                             & no-role   & 0.263*          & 0.281*            & 0.482***     & 0.077         & 0.317**               & 0.284 \\
        %     % \midrule
        %     % && \cline{3-8}
        %     \midrule
        %     \multirow{2}{*}{multi}  & client    & 0.457***        & 0.480***          & 0.562***     & 0.412***      & 0.561***              & 0.494 \\
        %                             & counselor & 0.332**         & 0.303**           & 0.478***     & 0.156         & 0.552***              & 0.364 \\

        %     \bottomrule
        % \end{tabular}
        \begin{tabular}{lllllllr}
            \toprule
                                            &                              & Open Mindedness & Conscientiousness & Extraversion & Agreeableness & Negative Emotionality & Avg.  \\
            Role                            & Model                        &                 &                   &              &               &                       &       \\
            \midrule
            \multirow[t]{3}{*}{participant} & Meta-Llama-3-8B-Instruct-BFI & 0.692***        & 0.554***          & 0.569***     & 0.448***      & 0.648***              & 0.582 \\
                                            & Qwen1.5-110B-Chat            & 0.457***        & 0.480***          & 0.562***     & 0.412***      & 0.561***              & 0.495 \\
                                            & Avg.                         & 0.574           & 0.517             & 0.566        & 0.430         & 0.605                 & 0.538 \\
            \cline{1-8}
            \multirow[t]{3}{*}{counselor}   & Meta-Llama-3-8B-Instruct-BFI & 0.652***        & 0.586***          & 0.550***     & 0.412***      & 0.539***              & 0.548 \\
                                            & Qwen1.5-110B-Chat            & 0.332**         & 0.303**           & 0.478***     & 0.156         & 0.552***              & 0.364 \\
                                            & Avg.                         & 0.492           & 0.445             & 0.514        & 0.284         & 0.546                 & 0.456 \\
            \cline{1-8}
            \multirow[t]{3}{*}{observer}    & Meta-Llama-3-8B-Instruct-BFI & 0.499***        & 0.560***          & 0.476***     & 0.357**       & 0.483***              & 0.475 \\
                                            & Qwen1.5-110B-Chat            & 0.367***        & 0.435***          & 0.451***     & 0.306**       & 0.523***              & 0.416 \\
                                            & Avg.                         & 0.433           & 0.498             & 0.463        & 0.332         & 0.503                 & 0.446 \\
            \cline{1-8}
            \multirow[t]{3}{*}{no-role}     & Meta-Llama-3-8B-Instruct-BFI & 0.455***        & 0.455***          & 0.421***     & 0.230         & 0.515***              & 0.415 \\
                                            & Qwen1.5-110B-Chat            & 0.183           & 0.236*            & 0.409***     & 0.090         & 0.349**               & 0.253 \\
                                            & Avg.                         & 0.319           & 0.345             & 0.415        & 0.160         & 0.432                 & 0.334 \\
            % \cline{1-8}
            \bottomrule
        \end{tabular}

    }
    % \caption{The pearson correlation between the predicted and actual BFI traits varies by role using Qwen1.5-110b-Chat~\cite{bai2023qwen}. The validity of predictions is notably enhanced by role-play. The client role shows the strongest correlation. * indicates p-value < 0.05, ** indicates p-value < 0.01, *** indicates p-value < 0.001. \YY{TODO: 1. Add name for the table. 2. Paragraph the description for clear understanding, show the importance of different role in the prediction, also explain the significance and reason for the difference. 3. Update data with the latest results, maybe add ``Llama3-8b-Instruct-BFI'' as well?}}
    \caption{Performance of Models in Predicting BFI Traits Across Different Roles. We evaluated the prediction of BFI traits across various roles (client, counselor, observer, and no-role) in real-world counseling sessions. Our model consistently surpasses Qwen1.5-110B-Chat~\cite{bai2023qwen}, particularly in the client role, where it achieves the highest average correlation. This underscores the effectiveness of role-based prompting strategies, with the client and counselor roles showing significantly higher prediction accuracies. The no-role condition exhibits the lowest performance, emphasizing the importance of contextual role-play in improving model predictions.}
    \label{tab:role_ablation}
\end{table*}

